Linear, or Non-Linear, That is the Question!

There were fierce debates on whether the non-linear embedding propagation of GCNs is appropriate to GCN-based recommender systems. It was recently found that the linear embedding propagation shows better accuracy than the non-linear embedding propagation. Since this phenomenon was discovered especially in recommender systems, it is required that we carefully analyze the linearity and non-linearity issue. In this work, therefore, we revisit the issues of i) which of the linear or non-linear propagation is better and ii) which factors of users/items decide the linearity/non-linearity of the embedding propagation. We propose a novel Hybrid Method of Linear and non-linEar collaborative filTering method (HMLET, pronounced as Hamlet). In our design, there exist both linear and non-linear propagation steps, when processing each user or item node, and our gating module chooses one of them, which results in a hybrid model of the linear and non-linear GCN-based collaborative filtering (CF). The proposed model yields the best accuracy in three public benchmark datasets. Moreover, we classify users/items into the following three classes depending on our gating modules' selections: Full-Non-Linearity (FNL), Partial-Non-Linearity (PNL), and Full-Linearity (FL). We found that there exist strong correlations between nodes' centrality and their class membership, i.e., important user/item nodes exhibit more preferences towards the non-linearity during the propagation steps. To our knowledge, we are the first who design a hybrid method and report the correlation between the graph centrality and the linearity/non-linearity of nodes. All HMLET codes and datasets are available at: https://github.com/qbxlvnf11/HMLET.

==> Linear or Non-Linear/algorithm_hmlet_end.tex <==
% \begin{algorithm}[t]
% % \small
% \footnotesize
% \caption{\oure }
% \label{algo:type_d} 
%   \begin{flushleft}
%       \textbf{Input:} user embedding $u_0$, item embedding $v_0$, linear layer $k$ and non-linear layer $k\prime$ \\
%       \textbf{Output:} residual $\hat{r}$, which will be used in the final prediction
%   \end{flushleft}
%     \begin{algorithmic}[1]
%         \STATE $e_u^{L_0^l}, e_u^{L_0^n} \leftarrow e_u $ \hfill \Comment{initial user embedding}
%         \STATE $e_v^{L_0^l}, e_v^{L_0^n} \leftarrow e_v $ \hfill \Comment{initial item embedding}

%         \REPEAT
%             \FOR{$i \leftarrow 1 \; \text{to} \; k$}
%                 \IF{$i \le (k-k\prime)$}
%                 \STATE $e_u^{L_{(i)}^l}, e_v^{L_{(i)}^l}  \leftarrow \test{AGG} (e_u^{L_{(i-1)}^l}, e_v^{L_{(i-1)}^l} )$
%                 \STATE $\hat{r} \mathrel{{+}{=}} e_u^{L_{(i)}^l} \odot\  e_v^{L_{(i)}^l}$

%                 \ELSIF{$i > (k-k\prime)$}
%                 \STATE $e_u^{L_{(i+k\prime)}^l} , e_v^{L_{(i+k\prime)}^l} \leftarrow \text{AGG}(e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l})$
%                 \STATE $e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n} \leftarrow \text{AGG}(e_u^{L_{(i-k\prime-1)}^n}, e_v^{L_{(i+k\prime-1)}^n})$
%                 % \STATE $e^{L^l} \leftarrow e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}$
%                 % \STATE $e^{L^n} \leftarrow e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n}$
%                 % \STATE $e^{L^g} \leftarrow GN(e^{L^l}, e^{L^n})$ \hfill \Comment{gating network phase}
%                 % \STATE $g \leftarrow GN(e^{L^l}, e^{L^n})$ \hfill \Comment{gating network phase}
%                 \STATE $g \leftarrow GN\left( (e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}), (e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n}) \right) $ \hfill \Comment{eq.(9)}
%                 % \STATE $e^{L^g} \leftarrow g \odot \text{stack}(e^{L^l}, e^{L^n})$
%                 \STATE $e_u^{L_{i-k\prime}^g}, e_v^{L_{i-k\prime}^g} \leftarrow g \odot \text{stack}\left( (e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}), (e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n}) \right)$
%                 % \STATE $e_u^{L_{i-k\prime}^g}, e_v^{L_{i-k\prime}^g} \leftarrow e^{L^g}$
%                 \STATE $\hat{r} \mathrel{{+}{=}} e_u^{L_{i-k\prime}^g} \odot\ e_v^{L_{i-k\prime}^g}$
%                 \ENDIF
%             \ENDFOR
%         \UNTIL{converge}
%     \end{algorithmic}
% \end{algorithm}
\SetInd{0.2em}{0.2em}
\begin{algorithm}[t]
% \footnotesize
\small
\SetAlgoLined
\DontPrintSemicolon
    Initialize $e_u^{L_0^l}, e_u^{L_0^n}, e_v^{L_0^l}, e_v^{L_0^n},$  linear layer $k$ and non-linear layer $k\prime$\;
    % $e_u^{L_0^l}, e_u^{L_0^n} \leftarrow e_u $ \;
    % $e_v^{L_0^l}, e_v^{L_0^n} \leftarrow e_v $ \;
    \While {the BPR loss $L$ is not converged}{
    \For{$i \leftarrow 1 \; \text{to} \; k$}{ 
        \uIf{$i \le (k-k\prime)$}{
            $e_u^{L_{(i)}^l}, e_v^{L_{(i)}^l} = \test{AGG} (e_u^{L_{(i-1)}^l}, e_v^{L_{(i-1)}^l} )$ \;
            $\hat{r} \mathrel{{+}{=}} e_u^{L_{(i)}^l}  \odot\  e_v^{L_{(i)}^l}$ \;
            
          }
          \Else{
             $e_u^{L_{(i+k\prime)}^l} , e_v^{L_{(i+k\prime)}^l} = \text{AGG}(e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l})$ \;
             $e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n} = \text{AGG}(e_u^{L_{(i-k\prime-1)}^n}, e_v^{L_{(i+k\prime-1)}^n})$ \;
             $g =$ \text{GN}$\big( e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}, e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n}  \big) $ \;
             $e_u^{L_{i-k\prime}^g}, e_v^{L_{i-k\prime}^g} = g \cdot \text{stack}\big( e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}, e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n} \big)$ \;
             $\hat{r} \mathrel{{+}{=}} e_u^{L_{i-k\prime}^g} \odot e_v^{L_{i-k\prime}^g}$ \;
          }
    }
    \Return $\hat{r}$ \;
}
\textbf{end}
\caption{\oure}
\label{algo:type_d} 
\end{algorithm}

==> Linear or Non-Linear/fig-degree-distribution.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
width=5cm,
% height=5cm, 
ylabel=Degree, xlabel=Nodes,
ymin=0, ymax=400,
nodes near coords align=vertical,
legend columns=3,
% legend pos=outer north,
legend cell align=left,
legend style={at={(0.50,1.2)},font=\footnotesize, anchor=center},
]
% FNL
\addplot[color=blue,mark=triangle,] file {results/FNL-degree.txt};\addlegendentry{FNL}
% PNL
\addplot[color=red,mark=oplus,] file {results/PNL-degree.txt};\addlegendentry{PNL}
% FL
\addplot[color=black,mark=square,] file {results/FL-degree.txt};\addlegendentry{FL}
% EAT
\end{axis}
\end{tikzpicture}
\vspace{-0.3cm}
\caption{Degree distribution on Gowalla.}\label{fig:degree}
\vspace{-0.3cm}
\end{figure}

==> Linear or Non-Linear/fig-rq2.tex <==
\begin{figure*}[t!]
\centering
\begin{tikzpicture}
\centering
\small
\begin{customlegend}[legend columns=4,legend style={align=center,draw=none,column sep=1.5ex}, legend cell align={left},
  legend entries={{\Etype}, {\Btype}, {\Ftype}, {\Dtype}}]
  \addlegendimage{area legend, draw=black, fill=black} %, postaction={pattern=grid}
  \addlegendimage{area legend, draw=black, fill=black!70} %, postaction={pattern=horizontal lines}
  \addlegendimage{area legend, draw=black, fill=black!40} %, postaction={pattern=vertical lines}
  \addlegendimage{area legend, draw=black, fill=black!10} %, postaction={pattern=dots}
  \end{customlegend}
\end{tikzpicture}

\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\amazon}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.0250, ymax=0.0300,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@20},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small },
        scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3},% rotate=20, 
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.0280)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.0280)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.0280)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.0300)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\yelp}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.0390, ymax=0.0440,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@20},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small }
        scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3}, % rotate=20, 
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.0431)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.0430)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.0430)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.0434)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\go}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.1190, ymax=0.1240,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@20},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small }, % rotate=20, 
       scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3},
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.1221)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.1221)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.1219)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.1231)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\vspace{-0.25cm}
\caption{Comparison ndcg (K=20) with all types of {\ours} on three public benchmarks.}
\label{fig:comparison-rq1}
\vspace{-0.25cm}
\label{fig:rq2}
\end{figure*}

\begin{figure*}[t!]
\centering
\begin{tikzpicture}
\centering
\small
\begin{customlegend}[legend columns=4,legend style={align=center,draw=none,column sep=1.5ex}, legend cell align={left},
  legend entries={{\Etype}, {\Btype}, {\Ftype}, {\Dtype}}]
  \addlegendimage{area legend, draw=black, fill=black} %, postaction={pattern=grid}
  \addlegendimage{area legend, draw=black, fill=black!70} %, postaction={pattern=horizontal lines}
  \addlegendimage{area legend, draw=black, fill=black!40} %, postaction={pattern=vertical lines}
  \addlegendimage{area legend, draw=black, fill=black!10} %, postaction={pattern=dots}
  \end{customlegend}
\end{tikzpicture}

\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\amazon}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.018, ymax=0.023,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@10},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small },
        scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3},% rotate=20, 
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.0209)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.0208)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.0208)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.0223)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\yelp}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.0290, ymax=0.0340,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@10},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small }
        scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3}, % rotate=20, 
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.0330)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.0328)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.0330)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.0332)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\go}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.1020, ymax=0.1060,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@10},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small }, % rotate=20, 
       scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3},
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.1046)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.1042)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.1043)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.1052)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\vspace{-0.25cm}
\caption{Comparison ndcg (K=10) with all types of {\ours} on three public benchmarks.}
\label{fig:comparison-rq2}
\vspace{-0.25cm}
\label{fig:rq2}
\end{figure*}

==> Linear or Non-Linear/macros.tex <==

\newcommand{\ie}{{\it i.e.,}}
\newcommand{\eg}{{\it e.g.,}}
\newcommand{\yc}[1]{\textcolor{blue}{#1}}
\newcommand{\js}[1]{\textcolor{green}{#1}}
\newcommand{\note}[1]{\textcolor{red}{#1}}
\newcommand{\go}{Gowalla}
\newcommand{\yelp}{Yelp2018}
\newcommand{\amazon}{Amazon-Book}
\newcommand{\light}{LightGCN}
\newcommand{\lrgccf}{LR-GCCF}
\newcommand{\ngcf}{NGCF}
\newcommand{\Etype}{\textsc{\textsf{HMLET}}(All)}
\newcommand{\Btype}{\textsc{\textsf{HMLET}}(Front)}
\newcommand{\Ftype}{\textsc{\textsf{HMLET}}(Middle)}
\newcommand{\Dtype}{\textsc{\textsf{HMLET}}(End)}

\newcommand{\ourf}{\textsc{\textsf{HMLET}}(Front)}
\newcommand{\ourm}{\textsc{\textsf{HMLET}}(Middle)}
\newcommand{\oure}{\textsc{\textsf{HMLET}}(End)}

\newcommand{\ours}{\textsc{\textsf{HMLET}}}
\newcommand{\geee}{\textsc{\textsf{GEE-E}}}

==> Linear or Non-Linear/sec-analysis.tex <==
\subsection{In-Detail Analysis}\label{sec:analysis}
In this subsection, we analyze in detail class ratio and the characteristics of each node selected by gating networks to confirm factors of determining which embedding propagation is effective. In order to analyze accurately, we utilize the results of {\Dtype} with the best accuracy among the all types of {\ours}.

\subsubsection {\bfseries{Node class and graph centrality}}\label{sec:node_class}
We first classify all nodes into three classes according to the type of the embedding selected by gating networks:

\begin{itemize}[leftmargin=*]
    \item {\bfseries Full-Non-Linearity (FNL)} is a class of nodes in which all embeddings selected by the gating networks are non-linear embeddings.

\item {\bfseries Partial-Non-Linearity (PNL)} is a class of nodes in which the embeddings selected by the gating networks are mixed with linear embeddings and non-linear embeddings.

\item {\bfseries Full-Linearity (FL)} is a class of nodes in which all embeddings selected by the gating networks are linear embeddings.
\end{itemize}

We next introduce three graph centrality measures
to clarify distinct characteristics of nodes that determine linear/non-linear embedding propagation:

\begin{itemize}[leftmargin=*]

\item {\bfseries Page Rank} 
~\cite{page1999pagerank} measures the relative importance of a node in the network. The more nodes with high rank are linked the more important node.

\item {\bfseries Betweenness Centrality} ~\cite{brandes2001centralitybet} measures the centrality of a node as an intermediary in the network. The more the node is included within the shortest path between all pairs of nodes in the network, the higher the betweenness centrality.

\item {\bfseries Closeness Centrality}~\cite{freeman1978centralitycls}
measures the centrality of a node by considering not only the direct connection information of the node but also the indirect connection information in the network. The more nodes are linked directly/indirectly the higher the closeness centrality.
\end{itemize}

\subsubsection {\bfseries{Analyzing relation of effectiveness to class ratio (RQ3)}}\label{sec:node_class_ratio}Table \ref{tab:class ratio} shows the class ratio of nodes on three datasets. Specifically, in the {\amazon} and {\yelp} datasets, most nodes were classified as FNL and PNL (about 47-8\%, 50-2\%), and very a few nodes were classified as FL (about 2\%). However, in the {\go} dataset, the ratio of FL nodes is about 12\%, which is relatively quite high compared to the other two datasets.

From the recommendation evaluation results in Table \ref{tab:comparison-rq1}, \ref{tab:comparison-rq2}  we found that the higher the ratio of FNL nodes, the better {\ours} methods perform than the linear GCN, LightGCN which shows the best performance among baselines. The results of analysis explain why remarkable performance improvements is observed in the Amazon dataset. Since the {\amazon} has the smallest FL node ratio, and the FNL ratios are high, the effectiveness is significantly improved when using non-linear embedding propagation together.

\subsubsection {\bfseries{Analyzing characteristics of class-specific nodes (RQ4).}}

We certainly confirm with previous experimental results that the linear/non-linear characteristics can be appropriately selected, although its ratio is changed depending on the dataset. We next analyze node attributes that determines which embedding is effective and use it to give insight for selection between linear embedding propagation and non-linear embedding propagation. 

Figure~\ref{fig:node_degree_distribution} shows the result of a degree distribution of nodes in the Amazon-Book dataset.\footnote{The other two datasets also show a similar trend, but due to page limit, only the result of the Amazon-Book dataset is shown here.} The x-axis represents nodes percentage ascending by degree at 10\% intervals, and the y-axis represents class ratio.
Figure~\ref{fig:box_plot} represents the graph centrality of the class-specific nodes in the {\amazon} dataset as a boxplot. From Figure~\ref{fig:node_degree_distribution} and Figure~\ref{fig:box_plot}, it can be seen that the degree and all centralities increase in the order of the FL, PNL, and FNL node in general. Here, we analyze the meaning of the above results for each class.

\begin{itemize}[leftmargin=*]
\item {\bfseries Full Non-Linearity (FNL) Nodes Attribute} 
 This node is either an active user or popular item with more direct/indirect interaction information (i.e., high degree and closeness centrality) and a high influence (i.e., high page rank and betweenness centrality) than nodes of other classes. They have a lot of direct/indirect interactions with other nodes and a strong influence, so they will receive a lot of information in the process of embedding propagation. However, since there is a lot of information being received, more informative and less informative nodes can coexist in predicting or presenting user preference. Therefore, it would be necessary to accurately distinguish nodes that are more informative to each of them through a non-linear operation.
 \item {\bfseries Full Linearity (FL) Nodes Attribute}
 This node is either a user or item that does not have much direct/indirect interaction information (i.e., low degree and closeness centrality) and a little influence (i.e., low page rank and betweenness centrality) compared to nodes of other classes. They do not have many direct/indirect interactions with other nodes and little influence, so the information they receive may mostly consist of information informative to them. Therefore, a simple linear operation (e.g., average) without a non-linear operation will be enough to well predict or represent the user's preference.
 \item {\bfseries Partial Non-Linearity (PNL) Nodes Attribute}
 This node, compared to nodes of other classes, is a user or item with neither too large nor too small direct/indirect interaction information (i.e., degree and closeness centrality between nodes in different classes) and influence (i.e., page rank and betweenness centrality between nodes in different classes). In other words, although they have many direct neighbors, there are few indirect neighbors connected to direct neighbors (because direct neighbors are mainly FL nodes), or even if there are few direct neighbors, their indirect neighbors could be many (because direct neighbors are mainly FNL nodes). Therefore, they need to perform non-linear or simple linear operations according to the information they receive from direct/indirect interactions during the process of embedding propagation.
\end{itemize}
 
 
 \begin{figure*}[t!]
\centering
% \usepackage{pgfplots}
\pgfplotsset{compat=1.8}
\usepgfplotslibrary{statistics}
\begin{subfigure}
\begin{tikzpicture}[scale=0.7]
  \begin{axis}[
    % [
    xlabel = {Page Rank},
    boxplot/draw direction=y,
    xtick={1,2,3},
    xticklabels={FNL, PNL, FL},
    x tick label style={font=\footnotesize, text width=2.5cm, align=center}
    ]
    \addplot+[
    boxplot prepared={
      lower whisker=1.18196E-06,
      lower quartile=3.3164E-06,
      median=4.8673E-06,
      upper quartile=8.05604E-06,
      upper whisker=1.51649E-05,
            %  average=8.0014E-06
    }, color = black, fill=black!60
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=1.16982E-06,
      lower quartile=3.14872E-06,
      median=4.54145E-06,
    %   average=6.02811E-06,
      upper quartile=6.63666E-06,
      upper whisker=1.18678E-05
    }, color = black, fill=black!40
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=1.21219E-06,
      lower quartile=2.68252E-06,
      median=3.61638E-06,
      upper quartile=5.16359E-06,
      upper whisker=8.87023E-06,
    %   average=4.76206E-06
    }, color = black, fill=black!20
    ] coordinates{};
    \end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}
\begin{tikzpicture}[scale=0.7]
  \begin{axis}[
    % [
    xlabel = {Betweenness Centrality},
    boxplot/draw direction=y,
    xtick={1,2,3},
    xticklabels={FNL, PNL, FL},
    x tick label style={font=\footnotesize, text width=2.5cm, align=center}
    ]
    \addplot+[
    boxplot prepared={
      lower whisker=0,
      lower quartile=1.5827E-06,
      median=4.66162E-06,
      upper quartile=1.51682E-05,
      upper whisker=3.55464E-05,
            %  average=3.04861E-05
    }, color = black, fill=black!60
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=0,
      lower quartile=1.28016E-06,
      median=3.50505E-06,
    %   average=1.31815E-05,
      upper quartile=9.67357E-06,
      upper whisker=2.22579E-05
    }, color = black, fill=black!40
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=0,
      lower quartile=6.21681E-07,
      median=1.83557E-06,
      upper quartile=5.4101E-06,
      upper whisker=1.24468E-05,
    %   average=7.84346E-06
    }, color = black, fill=black!20
    ] coordinates{};
    \end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}
\begin{tikzpicture}[scale=0.7]
  \begin{axis}[
    % [ylabel = {Closeness Centrality},
    xlabel ={Closeness Centrality},
    boxplot/draw direction=y,
    xtick={1,2,3},
    xticklabels={FNL, PNL, FL},
    x tick label style={font=\footnotesize, text width=2.5cm, align=center}
    ]
    \addplot+[
    boxplot prepared={
      lower whisker=0.206843691,
      lower quartile=0.239632048,
      median=0.24964174,
      upper quartile=0.261528364,
      upper whisker=0.294344759,
            %  average=0.250870241
    }, color = black, fill=black!60
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=0.205991771,
      lower quartile=0.235977482,
      median=0.245726143,
    %   average=0.245588375,
      upper quartile=0.255969292,
      upper whisker=0.285935459
    }, color = black, fill=black!40
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=0.15967715,
      lower quartile=0.21024025,
      median=0.230146713,
      upper quartile=0.244418274,
      upper whisker=0.295508604,
    %   average=0.227881812
    }, color = black, fill=black!20
    ] coordinates{};
    \end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Boxplots about centralities in Amazon-Book dataset. The Yelp2018 dataset shows a similar trend, but in the Gowalla dataset, the results of FL nodes are similar to the results of PNL nodes in the page rank and betweenness centrality.}
\label{fig:box_plot}
\end{figure*}

To make sure our interpretation is correct, we show the tendency of neighbors per each class. So, we calculate the similarity (i.e., cosine similarity) between the class-specific node and its direct neighbors using embeddings learned by {\Dtype}.
As can be seen from Table \ref{tab:similarity}, the mean of the similarity between class-specific nodes and their neighbors increases in the order of FNL, PNL, and FL node, and the variance increases in the order of FL, PNL, and FNL node.

From these results, we can confirm that FNL nodes' neighbors variously are consist of the more informative and less informative nodes (i.e., relatively low similarity means and high similarity variance) and FL nodes' neighbors mainly consist of informative nodes (i.e., high similarity mean and low similarity variance), and PNL nodes' neighbors have the characteristics of the FNL node and the FL node evenly (i.e., similarity mean and variance between nodes in different classes).

In this section, through multiple measures and experiments, we analyzed the characteristics of each of the user-item interactions that gating networks select linear or non-linear embedding propagation about. To the best of our knowledge, this is the first study to find out that linear and non-linear features in user-item interactions can coexist, and analyze what type of node each feature can occur in.

\begin{figure}
\centering
\begin{tikzpicture}[scale=0.7]
\begin{axis}[
    xlabel={Nodes ascending  by degree (at 10\% intervals)},
    % ylabel={Class-specific node ratio},
    % xlabel={Degree in ascending order (at 10\% intervals)},
    ylabel={Class ratio},
    xmin=0, xmax=90,
    ymin=0, ymax=80,
    xtick={0,10,20,30,40,50,60,70,80,90},
    xticklabels={10\%, 20\%, 30\%, 40\%, 50\%, 60\%, 70\%, 80\%, 90\%, 100\%,},
    ytick={0,10,20,30,40,50,60,70,80},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    mark options={solid}
]
\addplot[
   mark=*
    ]
    coordinates {
    (90,78.11895919) (80,75.20940871)
		(70,62.10739659) (60,54.9429539) (50,48.86218309) (40,42.92219384)
		(30,38.13066353) (20,34.57854787) (10,29.58106313) (0,24.81291262)
    };
\addplot[
    dashed,mark=triangle*
    ]
    coordinates {
    (90,11.70514673) (80,21.1389107)
		(70,31.2421691) (60,34.72602399) (50,35.97356713) (40,37.39357856)
		(30,37.8853709) (20,38.7649476) (10,37.60506112) (0,28.32400165)
    };
\addplot[
    dashed,mark=square*
    ]
    coordinates {
    (90,10.17589408) (80,3.651680582)
		(70,6.65043431) (60,10.33102211) (50,15.16424978) (40,19.68422761)
		(30,23.98396556) (20,26.65650453) (10,32.81387575) (0,46.86308574)
    };
    \legend{FNL,PNL,FL}
\end{axis}
\end{tikzpicture}
\caption{Node distributions in each class.}
\label{fig:node_degree_distribution}
\end{figure}



\begin{table}
  \caption{Similarity between the class-specific node and its direct neighbors}
  \label{tab:similarity}
  \begin{tabular}{cccc}
    \toprule
    Similarity & FNL & PNL & FL \\
    \midrule
    Mean & 0.6369 & 0.6449 & 0.7157 \\
    Variance & 0.0179 & 0.0162 & 0.0160 \\
  \bottomrule
\end{tabular}
\end{table}



\subsubsection{{\bfseries 

==> Linear or Non-Linear/sec-conclusions.tex <==
\section{Conclusions and Future Work}
In GCN-based recommender, we analyzed which linear/non-linear embedding propagation is appropriate and the characteristics of each embedding propagation systems by focusing on the existing GCN’s issues related to the use of linear embedding and non-linear embedding. Our proposed recommender system HEMLET can hybridize the linear and non-linear embedding propagation through the gating network in each layer by dynamically selecting appropriate embedding propagation. Our method shows the best accuracy in all datasets and we also presented in-depth analysis how linearity and non-linearity of nodes are decided in a network. Moreover, we classify users/items into three classes (Full-Linearity, Full-Non-Linearity, and Partial-Non-Linearity) depending on our gating network’s selections and find correlations between nodes’ centralities and their characteristics. We hope that our discovery encourages much follow-up research work.
\label{sec:conclusions}

==> Linear or Non-Linear/sec-evaluation.tex <==
\section{Experiments}\label{sec:experiments}

In this section, we evaluate our proposed approach via extensive experiments. We designed the experiments, aiming at answering the following key research questions (RQs):

{\begin{itemize}[leftmargin=*]
\item {\bfseries RQ1:} Does hybridizing the linear/non-linear embedding propagation provide more-accurate recommendations than either only using linear embedding or non-linear embedding?
\item {\bfseries RQ2:} 
Which architecture of our gating network is most effective in terms of recommendation accuracy?
\item {\bfseries RQ3:} 
How each embedding propagation affects to recommendation accuracy?
%\item {\bfseries RQ3:} 
%How embedding propagation ratio affects recommendation accuracy?
\item {\bfseries RQ4:} 
What are the characteristics of the nodes that affects to determination to use linear/non-linear embedding propagation?
\end{itemize}}

\begin{table}
  \caption{Statistics of public benchmark dataset}
  \label{tab:datasets}
  \begin{tabular}{ccccl}
    \toprule
    \textbf{Dataset} & \textbf{User \#} & \textbf{Item \#} & \textbf{Interaction} \# & \textbf{Sparsity} \\
    \midrule
    \textbf{\go} & 29,858 & 40,981 & 1,027,370 & 99.916\%\\
    \textbf{\yelp} & 31,668 & 38,048 & 1,561,406 & 99.870\%\\
    \textbf{\amazon} & 52,643 & 91,599 & 2,984,108 & 99.938\%\\
  \bottomrule
\end{tabular}
\end{table}

\begin{table*}[]
\caption{Comparison overall performance (K=20) with baseline models on three public benchmarks}
\label{tab:comparison-rq1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\toprule
Dataset  & \multicolumn{3}{c|}{Amazon-Book}                                                                                                                                                                       & \multicolumn{3}{c|}{Yelp2018}                                                                                                                                                                         & \multicolumn{3}{c|}{Gowalla}                                                                                                                                                                          \\ \hline
Metrics   & NDCG                                                       & Recall                                                     & Precision                                                  & NDCG                                                       & Recall                                                     & Precision                                                  & NDCG                                                       & Recall                                                     & Precision\\                  \hline\hline BPR      & 0.0181                                                              & 0.0307                                                              & 0.0065                                                              & 0.0289                                                              & 0.0476                                                              & 0.0062                                                              & 0.0847                                                              & 0.1341                                                              & 0.0203                                                              \\ \hline
WRMF     & 0.0242                                                            & 0.0405                                                            & 0.0085                                                            & 0.0402                                                              & 0.0645                                                              & 0.0145                                                              & 0.1007                                                              & 0.1538                                                              & 0.0243        \\ \hline
NGCF     & 0.0250                                                            & 0.0426                                                            & 0.0086                                                              & 0.0371                                                            & 0.0601                                                            & 0.0134                                                            & 0.1071                                                            & 0.1661                                                            & 0.0253                                                            \\ \hline
LR-GCCF  &  0.0213                                                           & 0.0361                                                            & 0.0077                                                            & 0.0351                                                            & 0.0581                                                            & 0.0129                                                            & 0.0989                                                            & 0.1545                                                            & 0.0240                                                           \\ \hline
{\light} & \textit{0.0283}                                                              & \textit{0.0484}                                                             & \textit{0.0099}                                                              & \textit{0.0420}                                                              & \textit{0.0678}                                                              & \textit{0.0152}                                                              & \textit{0.1212}                                                              & \textit{0.1870}                                                              & \textit{0.0288}                                                              \\ \hline\hline

\textbf{{\ours}}    & \textbf{\begin{tabular}[c]{@{}c@{}}0.0300\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0510\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0103\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0434\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0696\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0155\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.1231\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.1908\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0293\end{tabular}} \\ \hline 
\%Improv.      & 6.00\%                                                              & 5.37\%                                                              & 4.04\%                                                              & 3.33\%                                                              & 2.65\%                                                              & 1.97\%                                                              & 1.56\%                                                              & 2.03\%                                                             & 1.73\%                                                             \\ \hline
p-value     & 1.59E-37
                                                            & 1.71E-34
                                                            & 5.16E-36
                                                            &  5.57E-58
                                                             & 2.90E-39


                                                              & 1.61E-44
                                                              & 8.51E-25                                                              & 4.17E-131                                                              & 3.39E-27                      \\

\bottomrule\hline
\end{tabular}
\end{table*}

 \begin{table*}[]
 \caption{Comparison overall performance (K=10) with baseline models on three public benchmarks}
 \label{tab:comparison-rq2}
 \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
 \toprule
 Dataset  & \multicolumn{3}{c|}{Amazon-Book}                                                                                                                                                                       & \multicolumn{3}{c|}{Yelp2018}                                                                                                                                                                         & \multicolumn{3}{c|}{Gowalla}                                                                                                                                                                          \\ \hline
 Metrics   & NDCG                                                       & Recall                                                     & Precision                                                  & NDCG                                                       & Recall                                                     & Precision                                                  & NDCG                                                       & Recall                                                     & Precision\\                  \hline\hline BPR      & 0.0133                                                               & 0.0176                                                              & 0.0073                                                              & 0.0216                                                              & 0.0277                                                              & 0.0071                                                              & 0.0715                                                             & 0.0926                                                              & 0.0274                                                              \\ \hline
 WRMF     & 0.0181                                                            & 0.0236                                                            & 0.0097                                                            & 0.0308                                                              & 0.0386                                                              & 0.0170                                                              & 0.0864                                                              & 0.1084                                                              & 0.0336       \\ \hline
 NGCF     & 0.0186                                                          & 0.0250                                                            & 0.0099                                                           & 0.0280                                                            & 0.0350                                                            & 0.0155                                                            & 0.0916                                                            & 0.1162                                                            & 0.0351                                                             \\ \hline
 LR-GCCF  &  0.0158                                                           & 0.0215                                                            & 0.0087                                                            & 0.0264                                                            & 0.0349                                                            & 0.0150                                                            &  0.0841                                                            & 0.1081                                                           & 0.0327                                                          \\ \hline
 {\light} & \textit{0.0209}                                                             & \textit{0.0278}                                                             & \textit{0.0112}                                                              & \textit{0.0321}                                                              & \textit{0.0404}                                                              & \textit{0.0180}                                                              & \textit{0.1040}                                                              & \textit{0.1314}                                                             & \textit{0.0399}                                                              \\ \hline\hline

 \textbf{{\ours}}    & \textbf{\begin{tabular}[c]{@{}c@{}}0.0223\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0298\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0118\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0332\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0414\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0183\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.1052\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.1329\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0404\end{tabular}} \\ \hline 
 \%Improv.      & 6.27\%                                                              & 7.19\%                                                              & 5.35\%                                                              & 3.42\%                                                              & 2.41\%                                                              & 1.66\%                                                              & 1.15\%                                                              & 1.14\%                                                             & 1.25\%                                                             \\ \hline
 p-value     & 1.09E-39                                                             & 1.32E-38

                                                             &  4.72E-37                                                           & 1.31E-42
                                                               & 1.06E-30
                                                               & 1.44E-32                                                               & 7.83E-22                                                              & 9.79E-21                                                              & 1.21E-18
                       \\

 \bottomrule\hline
 \end{tabular}
 \end{table*}

\subsection{Experimental Setup}
\subsubsection{\bfseries{Datasets}}
For evaluation, we used three real-word datasets: \go, \yelp, and \amazon\ from various domains. They are all publicly available. Table~\ref{tab:datasets} shows the detailed statistics of the three datasets.

\begin{itemize}[leftmargin=*]
\item \textbf{\go} is a location-based social networking website where users share their locations by checking-in~\cite{liang2016modeling}. This dataset contains user-website interactions.

\item  \textbf{\yelp} is subset of small businesses and user data used in Yelp Dataset Challenge 2018. %\footnote{https://www.yelp.com/dataset/download}.
This dataset contains user-business interactions.

\item  \textbf{\amazon} is huge purchase history of Amazon users. {\amazon} has highest sparsity among these three public data sets. This dataset contains user-item interactions.
\end{itemize}

Following~\cite{Wang19NGCF}, we filtered out those users and items with less than ten interactions in all datasets (\ie\ a 10-core setting). For testing, we then split a dataset into training (80\%), validation (10\%), and test (10\%) sets in the same way as in ~\cite{Wang19NGCF}.


\subsubsection{\bfseries{Competing Methods}}
We compare the {\ours} with  2 baselines and 3 state-of-the-arts GCN-based models to verify its effectiveness.%\footnote{We performed the same as the experimental setup in~\cite{He20LightGCN}; thus, we did not compare with other neural network based methods that showed the lower accuracy than \light.}%
As the baselines, we compare ours with the traditional MF-based models:
\begin{itemize}[leftmargin=*]
    \item \textbf{WRMF}~\cite{Hu08WRMF} is a matrix factorization (MF) optimized by the \textit{weight alternating least square} (WALS) technique. It aims to minimize the errors between the real and predicted rating scores.
    \item  \textbf{BPRMF}~\cite{Rendle09BPR} is an MF optimized by the \textit{Bayesian personalized ranking} (BPR) loss. It aims to maximize the relative preference differences between a single item rated by a user and another single item that she has not rated.
\end{itemize}

Also, we compare ours with a state-of-the-art non-linear GCN and two liner GCNs:
\begin{itemize}[leftmargin=*]
    \item \textbf{\ngcf}~\cite{Wang19NGCF} is a non-linear GCN-based recommender system performing residual prediction.
    \item  \textbf{\lrgccf}~\cite{Chen20LRGCCF} is a linear GCN-based recommender system performing residual prediction.
    \item  \textbf{\light}~\cite{He20LightGCN} is a linear GCN-based recommender system performing residual prediction. This method differs from the LR-GCCF in that it removes all redundant parameters.
\end{itemize}

For MF-based methods, we used the implementations in the popular open-source NeuRec.%\footnote{https://github.com/wubinzzu/NeuRec}%
For GCN-based methods, we used the source codes provided by the authors~\cite{He20LightGCN,Chen20LRGCCF,Wang19NGCF}.
% % \subsubsection {\bfseries{Evaluation Metrics}}
% % \vspace{1mm}
% \note{(position?)\noindent\textbf{Evaluation Metrics.}
To evaluate the accuracy of \ours\ and the competing methods, we performed top-$k$ (20, 10)  recommendation using each method and measured its accuracy in terms of Precision, Recall, and \textit{normalized discounted cumulative gain} (NDCG), which are popularly used in a recommendation research~\cite{Wang19NGCF,Chen20LRGCCF,He20LightGCN}.

\subsubsection{\bfseries{Hyper-parameter Settings}}
For parameter tuning, we found the best settings in {\ours} and competing methods via extensive grid search with the validation set. The best setting found in {\ours} as follows: the number of the layer for linear GCN = 4, the number of the layer for non-linear GCN = 4({\Etype}) and 2({\Dtype}, {\Btype}, {\Ftype}), optimizer = Adam, learning rate $=0.001$, L2 regularization coefficient $\lambda = 1e-4$, mini-batch size $=2,048$, dropout rate $=0.4$. Also, for a fair comparison, we set embedding size for all GCN-based methods to the same dimensionality, $512$. In non-linear GCN, we use two nonlinear activation functions: Leaky-ReLU (negative slope = 0.01) and ELU ($\alpha$ = 1.0). We set temperature of Straight-Through Gumbel-Softmax~\cite{jang16categorical} for decay, original temperature as 0.7, minimum temperature as 0.01, and temperature decay value as 0.005.

\subsection{Performance Comparison}
% We first compare best type of {\ours} (\geee) with baseline models. Also, we compare each type of {\ours} to search most effective structure of proposed models.

\subsubsection{\bfseries{Comparison with competing methods (RQ1)}} \label{sec:comparison_competing_methods}
We conducted comparative experiments to show greater accuracy of {\ours} than that of 5 competing methods, \ie WRMF, BPRMF, NGCF, LRGCCF, and LightGCN.
Tables~\ref{tab:comparison-rq1} and ~\ref{tab:comparison-rq2} illustrate the result.
%\footnote{Due to space limitations, we omit the results for other top-$k$, which showed tendency similar to those in Tables~\ref{tab:comparison-rq1} and ~\ref{tab:comparison-rq2}. Please refer to all the results in [web link].} 
In Tables~\ref{tab:comparison-rq1} and ~\ref{tab:comparison-rq2}, the value in \textit{boldface} indicates the best accuracy in each column, and the value in \textit{italic} does the accuracy obtained from the best performer among all `competing' methods. 
Also, `\% Improve' indicates the degree of accuracy improvements from the best competing methods to \ours.
Lastly, we conduct $t$-tests with a 95\% confidence level to verify the accuracy differences between \ours\ and the competing methods.
The results in all measures and all datasets show that all $p$ values (see Tables~\ref{tab:comparison-rq1} and~~\ref{tab:comparison-rq2}) are below $0.05$, indicating the differences are statistically significant.

We summarize the results shown in Tables~\ref{tab:comparison-rq1} and ~\ref{tab:comparison-rq2} as follows. 
First, among five existing methods, we observe that {\light} consistently showed the best accruacy in all datasets. Also, we found that, unlike reported in~\cite{Chen20LRGCCF}, {\ngcf} always outperforms {\lrgccf} in our experiments performed grid search based on our dataset and setting. Second, {\ours} consistently and significantly provides the highest accuracy in all datasets and with all metrics. Specifically, for \amazon/\yelp/\go  \;datasets, {\ours} improve the NDCG@20 of \light, the best performer among the competing methods, by 6.00\%/3.33\%/1.56\%, respectively. Also, for three datasets, {\ours} improve the NDCG@10 of \light, the best performer among the competing methods, by 6.27\%/3.42\%/1.15\%, respectively.

The results indicate that (1) user-item interactions have only linear characteristics but also non-linear characteristics via selection ratio of gating networks as shown in Table~\ref{tab:gating_type} and (2) our gating networks appropriately selects linear/non-linear GCN by considering the inherent properties of users and items. Moreover, exploiting both linear and non-linear GCN is quite effective in predicting users' preferences on items, compared to only using liner GCN (\ie \lrgccf, and \light) or non-linear GCN (\ie \ngcf). We highlight that HMLET shows remarkable improvements in Amazon-Book dataset which is the largest one used in this paper. To discuss our observation, we will perform an in-depth analysis on this phenomenon in Section~\ref{sec:node_class_ratio}
% Similarly, {\ours} also demonstrates its effectiveness exhibiting improvements of Recall and Precision, by 5.37\%/2.65\%/2.03\% and 4.04\%/1.97\%/1.73\%. 
%\yc{Moreover, we highlight that \ours\ shows remarkable improvements in \amazon\ dataset which is the largest one used in this paper. 
%The results represent that as the complexity of user-item interactions increases, \ours\ is more effective. 
%In this sense, we conjecture that the large datasets contain quite a lot of both linearity and non-linearity.
%To demonstrate our claim, we will perform an in-depth analysis on this phenomenon in Section~\ref{sec:analysis}.}
% \note{(insert or not)Our model architecture is designed based on {\light} achieved best performances among existing models by using linear embedding propagation. We next add non-linear aggregating process allocated by gating networks to {\light}.}Our model architecture is consist of linear/non-linear embedding propagation process and gating networks allocating it. In this architecture, demonstration of being superior our model to linearity-based models means that appropriate allocation of linear/non-linear embedding propagation depending on the characteristics of each user-item interaction is more effective more than using only linear one. Moreover, If the decision criteria of allocating linearity and non-linearity will be clarified, we can choose an effective embedding propagation in recommender system, taking into account the characteristics of the data.
\input{fig-rq2}
\subsubsection{\bfseries{Comparison with each model structure (RQ2)}}
As mentioned in Section~\ref{sec:model-prop}, according to location of gating network, we designed four types of gating networks, \ie\ \Etype, \Btype, \Ftype, and \Dtype.
For RQ2, we first compare the accuracices of \ours s equipped with \Etype, \Btype, \Ftype, and \Dtype. Figures~\ref{fig:comparison-rq1} and ~\ref{fig:comparison-rq2} illustrate the result. %\footnote{Due to space limitations, we omit the results for other top-$k$, which showed tendency similar to those in Figures~\ref{fig:comparison-rq1} and ~\ref{fig:comparison-rq2}. Please refer to all the results in [web link].} 
In Figures~\ref{fig:comparison-rq1} and ~\ref{fig:comparison-rq2}, the x-axis represents the all types of {\ours}, and y-axis represents the NDCG@K (10, 20). 

We summarize the results shown in Figures~\ref{fig:comparison-rq1} and ~\ref{fig:comparison-rq2} as follows. First, {\Dtype} types is best performer among all types of {\ours}. Second, The performance of the types except for the {\Dtype} is similar. Specifically, the difference between {\Dtype} and other types is around 1\%/0.5\%/6\%, respectively, on {\go}, {\yelp}, {\amazon}. However, the performance difference of {\Etype}, {\Btype}, {\Ftype}, excluding {\Dtype}, is small as around 0.5\%.

The result indicate that (1) the effectiveness of the gating network depends on layer where the gating network exists, in other words, distance between the target embedding node and the neighboring node and (2) when embedding relationships with relatively long-distance (i.e. layer = 3, 4) neighbor nodes where embedding information can be vanishing due to noise, gating networks can be best utilized via selection of non-liner embedding information of short-distance (i.e. layer = 1, 2) node. As shown in Table~\ref{tab:gating_type}, each type has a 
quite different linear/non-linear embedding selection ratio. Best performer {\Dtype} is that utilization of non-linear embedding is high in layer 3, 4. This observation also applies to the second best-performing {\Etype}. When we perform an extended analysis on a dataset basis, we can observe similar results too. To discuss our observation, we will perform an in-depth analysis on this phenomenon in Section~\ref{sec:node_class_ratio}.

\begin{table*}
  \caption{Selection ratio of embedding propagation each type on {\amazon}}
  \label{tab:gating_type}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \toprule
    type of {\ours}&    \multicolumn{2}{c|}{layer 1}&    \multicolumn{2}{c|}{layer 2}&   
    \multicolumn{2}{c|}{layer 3}&   
    \multicolumn{2}{c|}{layer 4}\\   
    \hline
    embedding propagation & Lin. & Non. & Lin. & Non. & Lin. & Non. & Lin. & Non. \\
    \hline
    {\Etype} & 77.05\% & 22.95\% & 60.45\% & 39.55\% & 68.01\% & 31.99\% & 40.77\% & 59.23\% \\
    {\Btype} & 74.3\% & 25.7\% & 62.09\% & 37.91\% & 100\% & 0\% & 100\% & 0\%\\
    {\Ftype} & 100\% & 0\% & 63.03\% & 36.97\% & 72.41\% & 27.59\% & 100\% & 0\%\\
    {\Dtype} &100\% &0\%  &100\%  &0\%  &       5.19\% & 94.81\% & 49.55\% & 50.45\%\\
  \bottomrule
\end{tabular}
\end{table*}

\begin{table}
  \caption{Class ratio of nodes on three datasets}
  \label{tab:class ratio}
  \begin{tabular}{cccc}
    \toprule
    Class & Amazon-Book & Yelp2018 & Gowalla \\
    \midrule
    FNL & 46.78\% & 47.95\% & 27.49\% \\
    PNL & 51.77\% & 49.59\% & 60.84\% \\
    FL & 1.45\% & 2.46\% & 11.67\% \\
  \bottomrule
\end{tabular}
\end{table}

==> Linear or Non-Linear/sec-intro.tex <==
\section{Introduction}\label{sec:intro}
Recommender system is a personalized information filtering (IF) technology applied to many services, such as E-commerce, advertising, social media, and other many service platforms~\cite{covington2016deep, Ying18pinsage,yuan2020parameter}. The most popular recommender system, Collaborative Filtering (CF), provides personalized preferred items to users by learning user and item embeddings from their historical user-item interactions represented as a bipartite graph, etc ~\cite{8506344,10.1145/3285029,Koren2010,Y.Wu2016,He17NeuMF, Koren09MF,Wang19NGCF,Wang2014,Ebesu2018,Adomavicius2015,Yang2016}. %User-item interactions are represented as a bipartite graph~\cite{Wang19NGCF}.

One of the mainstream research directions in recommender systems is how to learn high-order connectivity of user-item interactions while filtering out noises. Recently, GCN-based CF became popular in recommender systems, because it has strong points to capture latent high-order connectivity between users and items. Since existing GCN is originally designed for graph classification tasks on attributed graph not recommender systems, however, two limitations had been raised out in that approach: training difficulty~\cite{Wu2019SGC,Chen20LRGCCF,He20LightGCN} and over-smoothing~\cite{chen2020measuring, li2018deeper}. Because of sparsity of user-item interactions bipartite graph, non-linear embedding propagation in GCN-based recommender systems generates excessive noise and hinders learning optimal embedding. Also, over-smoothing degrades performance by vanishing the connectivity information. To overcome these problems, usage of linear GCN (GCN based linear embedding propagation) was proposed instead of non-linear GCN (GCN based non-linear embedding propagation)~\cite{Chen20LRGCCF,He20LightGCN}. These methods effectively alleviate the two limitations and produce superior performance over non-linear GCN. Even if, linear GCN was proved for their effectiveness, when only one embedding propagation is used, it is not likely that we properly handle users/items with various characteristics. To us, it is still a question whether linear GCN is really superior to non-linear GCN and if so or not, which factors of graphs decide it.

To this end, we propose a \textbf{H}ybrid \textbf{M}ethod of \textbf{L}inear and non-lin\textbf{E}ar collaborating  fil\textbf{T}ering (\ours), a GCN-based recommender system with dynamically selecting between linear and non-linear embedding propagation considering each user/item's latent characteristics. {\ours} has the following features: i) we adopt a gating concept in each layer to decide between linear GCN and non-linear GCN. ii) we perform residual predictions, which mean embeddings from all layers are aggregated and used together for final predictions. Therefore, we let our gating neural network decide which of linear GCN or non-linear GCN is used for a certain node at a certain layer instead of relying on manually designed architectures.

To our knowledge, we are the first who attempts to combine linear and non-linear embedding propagation in a systematic way, i.e., our gating networks, which can be considered as relay switches, dynamically select between linear GCN and non-linear GCN operations in a layer. This mechanism can be considered as a sort of \emph{neural architecture search} for GCN-based CF. However, our proposed mechanism is much more sophisticated that it because we make decisions for each user/item and the overall GCN architecture can be varied from a certain node's perspective to another node's.

%hybridizes linear/non-linear embedding propagation to make it more flexible usage of two embeddings. Also, we use Gumbel-Softmax to make gating networks learnable.

We conduct performance comparison experiments using NDCG, Recall, and Precision and {\ours} shows the best performance on three benchmark datasets. Also, we define three classes of users/items depending on their preferences on linear GCN and non-linear GCN: FNL (Full-Non-Linearity), PNL (Partial-Non-Linearity), and FL (Full-Linearity). Finally, we analyze the class-specific characteristics of nodes and reveal an important relationship between nodes' roles in a network and their linearity/non-linearity. Contributions of our paper can be summarized as follow: {\begin{itemize}[leftmargin=*]
\item We propose HMLET, which adaptively selects the best propagation layer for a certain node at a certain layer.
\item We demonstrate the effectiveness of HMLET by showing that it marks the best accuracy in all three benchmark datasets.
\item We conduct in-depth analyses to show how linearity or non-linearity of nodes are decided.
\end{itemize}}


==> Linear or Non-Linear/sec-method.tex <==
\section{Proposed Approach}\label{sec:method}
% \usepackage{tabularx} % <-- new

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{img/overview.pdf}
  \caption{Overview of \ours. One can consider our gating network as a relay switch between linear and non-linear layers. While calculating an embedding for a user or an item, therefore, our gating network learns the optimal selection providing the best prediction accuracy, e.g., it selects linear $\rightarrow$ non-linear $\rightarrow$ linear for some user or item while it selects a totally different sequence for other user or item.}\label{overview}
\end{figure*}

In this section, we propose our method \ours. Its key concept is to adopt gating between linear and non-linear propagation layers. In other words, we prepare both linear and non-linear propagation layers but let our gating network with the Gumbel-Softmax decide which one to use in each layer. Table~\ref{table:notations} summarizes a list of notations used in this paper and Figure~\ref{overview} illustrates an overview of \ours.
Specifically, given a user-item pair $(u,v)$, \ours\ first builds a dense embedding of the user $u$ (resp. the item $v$) through the embedding layer (Section 3-1).
After that, the embedding of the user $u$ (resp. the item $v$) is propagated to its neighbors through propagation layers (Section 3-2-1).
Here, \ours\ selects either a linear or a non-linear embedding in consideration of  inherent characteristics with respect to the user $u$ (resp. the item $v$) in each layer (Section 3-2-2). 
To this end, we use a gating network based on the Gumbel-Softmax to select a better embedding for each user/item between linear and non-linear ones. 
The Gumbel-Softmax learns an optimal categorical distribution about the selection and lets the gating network select correctly between the linear and non-linear embedding propagation.
In order to predict each user's preference on each item, the user embedding and item embedding selected by the gating network in each layer is aggregated and we perform their dot-product for prediction.

\begin{table}[t]
    \caption{Notations used in this paper}
    \small
    \centering
    \renewcommand{\arraystretch}{1.7}
    \begin{tabular}{c|l}
        \toprule
        \textbf{Notation}                 & \textbf{Description}    \\
        \midrule
        $k$, $k'$, $k''$  & number of layers for liner, non-linear, and gating network \\
        \hline
        $\bm{e}_{u}^{L^l_{i}}$, $\bm{e}_{v}^{L^l_{i}}$     & $u$'s, $v$'s embedding at $i$-th linear layer      \\
        \hline
        $\bm{e}_{u}^{L^n_{i}}$, $\bm{e}_{v}^{L^n_{i}}$       & $u$'s, $v$'s embedding at $i$-th non-linear layer  \\
        \hline
        $\bm{e}_{u}^{L^g_{i}}$, $\bm{e}_{v}^{L^g_{i}}$        & $u$'s, $v$'s embedding selected by gating network at $i$-th layer\\
        \hline
        $d$    & size of embedding dimension    \\
        \hline
        $m$, $n$    & the number of users/items     \\
        \hline
        $\hat{r}_{uv}$    & user $u$'s final preference on item $v$    \\
        \hline
        $\mathcal N_u$, $\mathcal N_v$    & set of items rated by user $u$ and users who rated item $v$ \\
        \bottomrule
    \end{tabular}
    \label{table:notations}
\end{table}

\subsection{Embedding Layer}\label{subsec:embedding}

First, \ours\ represents users (resp. items) as latent vectors through the embedding layer. 
As shown in Figure~\ref{fig:embedding}, we define the embedding layer for users and items as a selection over $\bm{P}\in \mathbb{R}^{m\times d}$ and $\bm{Q}\in \mathbb{R}^{n\times d}$, respectively. 
Given a one-hot vector of a user $\bm{u}$ (resp. an item $\bm{v}$), the embedding layer maps it into a row of $\bm{P}$ (resp. $\bm{Q}$), yielding an embedding $\mathbf e_u$ (resp. $\mathbf e_v$).

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{img/embedding.pdf}
    \caption{Embedding Layer.}\label{fig:embedding}
\end{figure}

%% Insert the formation of Linear GCN, Non-linear GCN 

\subsection{Propagation Layer}\label{sec:model-prop}
\ours\ propagates the embedding $e_u$ (resp. $e_v$) of each user $u$ (resp. item $v$) through propagation layers. 
In this subsection, we describe the propagation process. Eq.~\eqref{eqn:propagate} describes the process of capturing high-order proximity. 
In Section 3-2-1, we formally define the linear-GCN and non-linear-GCN used in this paper.
In Section 3-2-2, we present our gating network that appropriately selects between them in each layer.

\subsubsection{\bfseries{Graph convolution}}
% \paragraph{\textbf{Graph convolution}}
First, embedding vectors are aggregated (AGG) as follows:
\begin{equation}
    \label{eqn:propagate}
    \begin{split}
    \bm{e}_{u}^{L_{i+1}} = AGG( \bm{e}_u^{L_i}, \lbrace \bm{e}_v^{L_i}: v\in \mathcal N_u \rbrace,\\
    \bm{e}_{v}^{L_{i+1}} = AGG( \bm{e}_v^{L_i}, \lbrace \bm{e}_u^{L_i}: u\in \mathcal N_v \rbrace).
    \end{split}
\end{equation}
where $\bm{e}_u^{L_i}$ and $\bm{e}_v^{L_i}$ indicate user $u$'s embedding and item $v$'s embedding at $i\text{-th}$ layer, respectively. 
That is, $(i+1)\text{-th}$ layer updates $u$'s embedding $\bm{e}_u^{L_{i+1}}$ by aggregating the embeddings of $u$ and $v$ rated by $u$ from $i\text{-th}$ layer.
Similarly, we do the same thing for $\bm{e}_v^{L_{i+1}}$.

Recently, a linear GCN~\cite{He20LightGCN} has been proposed to solve the over-smoothing problem of a non-linear GCN by removing a feature transformation and non-linear activation functions, and it shows better performance than existing non-linear GCN. In \ours, we adopt the linear layer definition of \light. The linear embedding propagation of \light\ is performed as follows:
\begin{equation}
    \begin{split}
    \bm{e}_{u}^{L^l_{i+1}} = \mathop{\mathlarger{\sum}}_{v\in  \mathcal N_u} \frac{1}{\sqrt{\vert \mathcal N_u \Vert \mathcal N_v \vert}} \bm{e}_{v}^{L^l_{i}},\\
    \bm{e}_{v}^{L^l_{i+1}} = \mathop{\mathlarger{\sum}}_{v\in \mathcal N_v} \frac{1}{\sqrt{\vert \mathcal N_v \Vert \mathcal N_u \vert}} \bm{e}_{u}^{L^l_{i}}.
    \end{split}
\end{equation}
where $\bm{e}_{u}^{L^l_{i}}$ and $\bm{e}_{v}^{L^l_{i}}$ indicate user and item embeddings at $i\text{-th}$ layer by \light, respectively. $\frac{1}{\sqrt{\vert \mathcal N_u \Vert \mathcal N_v \vert}}$ is a symmetric normalization term that prevents the scale of embedding from increasing as propagation goes on.

For non-linear embedding propagation, we design a variant of linear embedding propagation of \light\ by adding a non-linear activation function. Its propagation is preformed as follows:
\begin{equation}
    \begin{split}
    \bm{e}_{u}^{L^n_{i+1}} = \phi ( \mathop{\mathlarger{\sum}}_{v\in \mathcal N_u} \frac{1}{\sqrt{\vert \mathcal N_u \Vert \mathcal N_v\vert }}  \bm{e}_{v}^{L^n_{i}} ),\\
    \bm{e}_{v}^{L^n_{i+1}} = \phi ( \mathop{\mathlarger{\sum}}_{v\in \mathcal N_v} \frac{1}{\sqrt{\vert \mathcal N_v \Vert \mathcal N_u\vert }}  \bm{e}_{u}^{L^n_{i}} ).
    \end{split}
\end{equation}
where $\phi$ is a non-linear activation (e.g., ELU, Leaky ReLU, etc.). 

Note that \ours\ use both the linear and non-linear GCN intercorrelated through gating networks which will be described in next subsection.
% Therefore, we can employ any GCN models under \ours\ (\ie\ model-agnostic). 
% In this sense, when a \textit{linear/non-inear GCN} with better performance are available, \ours\ can simply replace the current GCN with that model, thereby improving the accuracy of recommendation.

\subsubsection{\bfseries{Gating network}}
% \paragraph{\textbf{Gating network}} 
Now, we have the linear and non-linear embeddings obtained from $i\text{-th}$ layer.
In this case, as mentioned earlier, linear or non-linear features may coexist in user-item interactions.
Therefore, we should appropriately select linear/non embedding that represents latent space of each user/item.
Toward this end, we design a gating network that adaptively selects either a linear or non-linear embedding by analyzing inherent characteristics of a given user or item.

Figure~\ref{fig:gating} shows the overall architecture of our gating network.
In the case of users, given both the linear and non-linear embeddings, denoted $\bm{e}_{u}^{L^l_{i}}$ and $\bm{e}_{u}^{L^n_{i}}$, respectively, of a user $u$, our gating network selects the best one, denoted as $\mathbf e_{u}^{L^g_{i}}$, and then propagate it to next layer.
Similarly, the gating network selects the best embedding propagation for each item.
% Note that \ours\ here selects one embedding each from every layer, rather than the specific layers.
The intuition behind this technique is that the embedding of each user (resp. item) may consist of both linear and non-linear components.
We formally define the process of performing the gating network in each layer as follows:
\begin{equation}
    \begin{split}
        \bm{g} &= \text{GN}(\bm{e}_{u}^{L^l_{i}},\bm{e}_{v}^{L^l_{i}},\bm{e}_{u}^{L^n_{i}},\bm{e}_{v}^{L^n_{i}}), \\
        \bm{e}_{u}^{L^g_{i}},\bm{e}_{v}^{L^g_{i}} &= \bm{g} \cdot \; \text{stack}(\bm{e}_{u}^{L^l_{i}},\bm{e}_{v}^{L^l_{i}},\bm{e}_{u}^{L^n_{i}},\bm{e}_{v}^{L^n_{i}}),
    \end{split}
\end{equation}
where GN indicates the gating network in Algorithm ~\ref{alg:gating}. The input embeddings are concatenated and then passed to a MLP (multi-layer perceptron). The result of the MLP is a logit vector $\bm{l}$, an input for the STGS.
The logit vector $\bm{l}$ corresponds to $\log \bm{\pi} $ explained in Section~\ref{subsec:gumbel}. $\bm{g}$, the output of GN, represents a linear or non-linear selection by the gating network.
The finally selected embedding $e_u^{L_{i}^g }$, $e_v^{L_{i}^g }$ by the gating network can be calculated by the dot-product at the end.

\begin{algorithm}[t]
  \small
  \DontPrintSemicolon
  \SetAlgoLined
  \KwIn{User and item embeddings}
  \SetKwFunction{FMain}{GN}
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{ $\bm{e}_{u}^{L_i^l}, \bm{e}_{v}^{L_i^l}, \bm{e}_{u}^{L_i^n}, \bm{e}_{v}^{L_i^n}$}}{
        $\bm{e}_{\text{concat}} \gets [ \bm{e}_{u}^{L_i^l}, \bm{e}_{v}^{L_i^l}, \bm{e}_{u}^{L_i^n}, \bm{e}_{v}^{L_i^n} ]$ \\
        $\bm{l} \gets $\text{MLP}$(\bm{e}_{\text{concat}})$\; \\
        $\bm{g} \gets $\text{STGS}$(\bm{l}, \tau)$\; \\
  }
  \KwRet $\bm{g}$\;
  \caption{Gating Network}\label{alg:gating}
\end{algorithm}

 \begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{img/gating3.pdf}
     \caption{The overall architecture of our gating network.}\label{fig:gating}
 \end{figure}

% Given both $\mathbf(e_{u}^{L^l_{i}}$ (resp. $e_{v}^{L^l_{i}}$) and $\mathbf (e_{u}^{L^n_{i}},e_{v}^{L^n_{i}})$ of a user $u$ 
% at $i$-th layer, our gating network selects a embedding, $\mathbf(e_{u}^{L^g_{i}},e_{v}^{L^g_{i}})$ , through the gating network, 
% % which is the output embedding $\mathbf(e_{u}^{L^l_{i}},e_{v}^{L^l_{i}})$, $\mathbf (e_{u}^{L^n_{i}},e_{v}^{L^n_{i}})$ of each $i-$th layer. 
% The selected embedding $\mathbf(e_{u}^{L^g_{i}},e_{v}^{L^g_{i}})$ is used as the input of the next $(i+1)\text{-th}$ layer. The intuition behind this model is that the embedding of each user (resp. item) is that different features(linear or non-linear) are aggregated and updated for each $i-$hop neighbor.


However, in the case of non-linear layers, an over-smoothing problem occurs when the number of layers is large. 
To address this problem, we further design variants of the gating network, which can be used when the number of linear layers is more than the number of non-linear layers.
As shown in Figure \ref{fig:types}, there can be three variants, denoted as \ourf, \ourm, and \oure,  depending on the location of the non-linear layer. 
% Each of the variants is presented in .
Specifically, \ourf, \ourm, and \oure\ employ the gating network at initial layers, middle layers, and last layers, respectively. 
First, \ourf\ focuses on the fact that GCNs are highly influenced by near neighborhood~\cite{tang15line}, such as 1-hop and 2-hop neighbors. 
Therefore,  \ourf\ performs the gating network in the front and then only uses the linear propagation layer.
% can be learned by selecting embedding better than linear embedding in the beginning. 
%Figure \ref{fig:types}-Type C is a model that reinforces embedding by using the embedding of a linear model that has been proven to have good performance for the initial embedding and the last embedding, and selecting linear embedding and non-linear embedding in the middle. 
Next, \ourm\ only uses linear embedding with good performance in the front and then performs the gating network at the end.
% Finally, Figure \ref{fig:types}-Type D, linear embedding with good performance is used for initial embedding, and linear embedding and non-linear embedding are selected only at the end. 
The intuition behind \oure\ is that we fine-tune embeddings learned by linear layers at the end --- our experiments and analyses show that \oure is the best among the three variations of the proposed method. The algorithm of our most effective \oure\ is in Algorithm~\ref{algo:type_d}.
% It can be said that fine-tuning was performed using the \textit{non-linear GCN} in the \textit{linear GCN}.
%\textit{linear GCN} with good performance is used, and the non-linear model and the linear model are considered together at the end, further reinforcing embedding that is not well learned in the linear model. That is, it is the same as learning through a linear model and fine-tuning using a non-linear model.

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{img/types.pdf}
    \caption{Three variants of our gating network.}\label{fig:types}
\end{figure} 

% Among the variants, we predict that the \ourm\ that reinforces embedding by using a \textit{linear GCN} with good performance at the beginning and a \textit{non-linear GCN} at the last embedding will be the best. 
% In Section~\ref{sec:eval}, we confirm that \ourm\ is the most effective in terms of recommendation accuracy, compared to other variants.

\input{algorithm_hmlet_end}

\subsection{Prediction Layer}\label{subsec:prediction}
After propagating through all $k$ layers, we predict each user's preference for each item. To this end, we create a dot-product value of the selected embeddings by our gating network in each layer and use the residual prediction as follows:
\begin{align}\begin{split}\label{eq:aaa}
    \hat{r}^{i}_{uv} =& \; \mathbf  e_{u}^{L_{i}} \odot \mathbf  e_{v}^{L_{i}},\\
    \hat{r}_{uv} =& \mathop{\mathlarger{\sum}}^k_{i=0} \hat{r}^{i}_{uv}.
\end{split}\end{align}
In the previous GCN-based recommendation system research, only the last embedding was used to predict, but in \ours, the above residual prediction $\hat r_{uv}$ is used. This residual prediction can produce good performance by using not only the last embedding but also the early embedding.
In summary, \ours\ predicts users' preferences on the items by considering both linear embedding and non-linear embedding based on the residual prediction.
% and all hops.

\subsection{Training Method}\label{subsec:opt}

For training \ours, we employ the Bayesian personalized ranking (BPR) loss, denoted $L$, which is popularly used in many CF method\cite{Rendle09BPR}. 
The BPR loss is as follows:
% \begin{equation}
%     \begin{split}
%     \mathbf L(R,\hat{R}) = - \mathop{\mathlarger{\sum}}^M_{a=1} \mathop{\mathlarger{\sum}}_{ (i,j) \in D_a} \ln \sigma(\hat{r}_{ai} - \hat{r}_{aj}) + \lambda\lVert \mathbf{\Theta_1} \rVert ^2,
%     \end{split}
% \end{equation}

\begin{equation}
    \begin{split}
    \mathbf L(R,\hat{R}) = - \mathop{\mathlarger{\sum}}^M_{u=1} \mathop{\mathlarger{\sum}}_{i\in N_u} \mathop{\mathlarger{\sum}}_{j\notin N_u}  \ln (\sigma(\hat{r}_{ui} - \hat{r}_{uj})) + \lambda\lVert \mathbf{\Theta_1} \rVert ^2
    \end{split}
\end{equation}
where $\sigma$ is the sigmoid function. $ \Theta_{1}$ is the embedding of the $0-$th layer, and $\lambda$ controls the $L_2$ regularization strength. We use each observed user-item interaction as a positive instance and then conduct the negative sampling strategy. 

Also, we employ STGS for smooth optimization of the gating network. We can train the network with annealing temperature, and we use the temperature decay for each epoch. Furthermore, we train a model that shows outstanding performance through the optimal temperature range and decay value.



% $ D_a = \{ (i,j) \vert i \in R_{a} \land j \in V-R_{a} \} $ denotes the pairwise training data for $a$ with $R_a$ represents the itemset that $a$ positively shows feedback. 

==> Linear or Non-Linear/sec-relatedwork.tex <==
\section{Related Work}\label{sec:related}
In this section, we briefly review traditional recommender systems including GCN-based methods and present Gumbel-Softmax used in our proposed methods.

\subsection{Recommender Systems}
Traditional recommender systems have focused on matrix factorization (MF) techniques ~\cite{Koren09MF}. Typical MF-based methods include BPR~\cite{Rendle09BPR} and WRMF~\cite{Hu08WRMF}. These MF-based methods simply learn relationships between users and items via dot products. Therefore, they have limitations in considering potential complex relationships between users and items inherent in user-item interactions~\cite{He17NeuMF}. To overcome these limitations, deep learning (DL) (e.g., Autoencoder \cite{kingma2013auto,rezende2014stochastic}, graph convolutional networks (GCNs)~\cite{Bruna2014,Defferrard2016,kipf2017semi,Wu2019SGC,Atwood2015,Gilmer2017,Hamilton2017,Velickovic2018,Gao2018}) based recommender systems have been proposed in recommendation domains to effectively learn those non-linear relationships between users and items ~\cite{Wang19NGCF,Ying18pinsage,liu08eigenrank,Rianne17GCMC}.

Recently, recommender systems~\cite{Wang19NGCF,Ying18pinsage,Rianne17GCMC} using GCNs are getting much attention. GCN-based methods can effectively learn the behavioral similarity between users and items by 'directly' capturing the collaborative signals inherent in user-item interactions~\cite{Wang19NGCF}. Typical GCN-based methods include GC-MC~\cite{Rianne17GCMC}, PinSage~\cite{Ying18pinsage}, and NGCF~\cite{Wang19NGCF}.

Generally, GCN-based methods model user-item interactions as a user-item bipartite graph and then perform the following three steps:

{\bfseries (Step 1) Embedding Layer:} We randomly set the initial embedding $e^0$ of all users $u$ and items $v$.
\begin{equation}
    \begin{split}
    \mathbf  e_{u}^{0}, e_{v}^{0} \in \mathbb {R}^{d}
    \end{split}
\end{equation}
where $d$ denotes the embedding size.

{\bfseries (Step 2) Propagation Layer:} Given $k$ layers, the embedding of a user node $u$ (resp. an item node $v$) in $i$-th (i.e., 1≤$i$≤$k$) layer is updated based on the embeddings of $u$ (resp. $v$) and its neighbors $N_u$ (resp. $N_v$) in ($i$-1)-th layer.

\begin{equation}
    \begin{split}
    \mathbf  e_{u}^{i} = \sigma ( \Sigma_{v\in N_u} e_v^{i-1} W_{i-1} ), \\
    \mathbf  e_{v}^{i} = \sigma ( \Sigma_{u\in N_v} e_u^{i-1} W_{i-1} ).
    \end{split}
\end{equation}

where $\sigma$ denotes a non-linear activation function (e.g., $ReLU$), and $W_{i-1}$ is a trainable transformation matrix. Some methods also include a self-embedding in the ($i$-1)-th layer (i.e., $e_{u}^{i-1}$ or $e_{v}^{i-1}$, respectively) during the aggregation process.

{\bfseries (Step 3) Prediction Layer:} The preference of user $u$ for item $i$ is predicted using the dot-product between the user $u$ and item $i$ embeddings of the last layer $k$ (i.e., $e_{u}^{k}$ and $e_{v}^{k}$).

\begin{equation}
    \begin{split}
    \hat{r}_{uv} = e_{u}^{k} \odot e_v^k
    \end{split}
\end{equation}

However, these GCN-based methods have two limitations: (L1) Training Difficulty ~\cite{Wu2019SGC,Chen20LRGCCF,He20LightGCN} and (L2) Over-Smoothing (i.e., indistinguishable embeddings of nodes) ~\cite{chen2020measuring,li2018deeper}. First, (L1) is caused by their ~\cite{Rianne17GCMC,Ying18pinsage,Wang19NGCF} use of a non-linear activation function in the propagation step. Specifically, the non-linear operation of the activation function complicates the propagation layer step and furthermore this operation is repeatedly performed whenever a layer is stacked over. Thus, they suffer from training difficulty with non-linear activation functions for large-scale user-item bipartite graphs ~\cite{Wu2019SGC,chen2020measuring,li2018deeper}.

Next, (L2) is caused as they ~\cite{Rianne17GCMC,Ying18pinsage,Wang19NGCF} use only the embeddings updated through the last layer in the prediction layer. Specifically, as the layer becomes deeper, the embedding of each node will receive more of the embeddings of its neighborhood. As a result, the embedding of each node in the last layer becomes similar to the embedding of many directly/indirectly connected nodes, resulting in the loss of uniqueness~\cite{Chen20LRGCCF,chen2020measuring,li2018deeper}. This phenomenon prevents traditional GCN-based methods from effectively utilizing information of high-order neighborhood. Empirically, this is also shown by the fact that many GCN-based methods show better performance when using only two layers than using more than two.

Recently, LR-GCCF~\cite{Chen20LRGCCF} and LightGCN~\cite{He20LightGCN}, which are GCN-based recommender systems to alleviate both (L1) and (L2), have been proposed. First, to alleviate (L1), they perform linear embedding propagation without using a non-linear activation function in the propagation layer step. Also, to mitigate (L2), they aggregate the embeddings of the last layer as well as the embeddings of all other earlier layers for prediction. After that, they perform residual predictions~\cite{Chen20LRGCCF, He20LightGCN}, which predict each user's preference for each item based on the aggregated embedding. In~\cite{Chen20LRGCCF,He20LightGCN}, the authors demonstrated that a GCN structure with linear embedding propagation and residual prediction can significantly improve the recommendation accuracy by successfully addressing (L1) and (L2).

\begin{table*}
  \caption{GCN-based Recommender Systems}
  \label{tab:GCNs}
  \begin{tabular}{ccccccc}
  \toprule
  & GC-MC~\cite{Rianne17GCMC} & PinSage~\cite{Ying18pinsage} & NGCF\cite{Wang19NGCF} & LR-GCCF~\cite{Chen20LRGCCF} & LightGCN\cite{He20LightGCN} & \textbf{Ours}
\\ \midrule
Non-Linear Embedding Propagation & O & O & O & X & X & O \\
Linear Embedding Propagation & X & X & X & O & O & O \\
Residual Prediction & X & X & O & O & O & O\\
\bottomrule
\end{tabular}
\end{table*}

In summary, GCN-based recommender systems can be categorized by, as shown in Table \ref{tab:GCNs}, propagation and prediction methods. Here, we note that they consider only one of the linear/non-linear characteristics of user-item interactions. However, we conjecture that user-item interactions are neither only linear nor only non-linear, for which we will conduct in-depth analyses in Section~\ref{sec:analysis}. Therefore, in this paper, we propose a \textbf{H}ybrid \textbf{M}ethod of \textbf{L}inear and non-lin\textbf{E}ar collaborating fil\textbf{T}ering method (\ours, pronounced as Hamlet), which consider both two disparate characteristics for selecting proper embedding propagation every layer.
\subsection{Gumbel-Softmax}\label{subsec:gumbel}
The Gumbel-max trick \cite{Gumbel54,Maddison14sampling} provides a way to sample a one-hot vector from a categorical distribution with class probabilities $\bm{\pi}$:
\begin{equation}
    \label{eqn:Gumbel-max}
   \bm{z}=one\_hot(\arg \max\limits_{\substack{i}}[g_i+log\pi_i])
\end{equation}
where $g_1...g_k$ are samples drawn from the unit Gumbel distribution $Gumbel(\bm{0},\bm{1})$. The argmax operator prevents gradients flowing through the Gumbel-max, because it gives zero gradients irrespective of how $\pi$ was created, which loss function is used, and so on. To this end, the Gumbel-Softmax~\cite{jang16categorical} function generates a sample $\bm{y}$ that approximates $\bm{z}$ via the reparameterization trick defined as follow:
\begin{equation}
    \label{eqn:Gumbel-Softmax}
    y_i=\frac{\exp \left(\left(\log \left(\pi _i\right)+g_i\right)/\tau \right)}{\sum _{j=1}^k\exp \left(\left(\log \left(\pi _j\right)+g_j\right)/\tau \right)}
\end{equation}
where $y_i$ is $i-$th component of the vector $\bm{y}$, and $\tau$ is a temperature that determines how closely the function approximates the sample $\bm{\pi}$. However, the Gumbel-Softmax is challenging to use if it needs to be sampled into discrete values because, when the temperature is high, the Gumbel-Softmax output is not categorical. To solve this problem Straight-Through Gumbel-Softmax (STGS) can be used. STGS always generates discrete outputs while letting the gradients flow through $y_i$, even when the temperature is high. This makes the network learnable while annealing the temperature.

This Gumbel-Softmax has been widely used to learn optimal categorical distributions. One such example is \emph{network architecture search (NAS)} ~\cite{hu2020neural,wan2020fbnetv2,chang2019differentiable,wu2019fbnet,he2020milenas,xie2018snas,li2020neural,hu2020dsnas}. In NAS, we let an algorithm find optimal operators (among many pre-determined candidates prepared by user) and their connections. All these processes can be modeled by generating optimal one-hot (or multi-hot) vectors and the Gumbel-Softmax is used~\cite{jang16categorical}. Another example is a multi-generator-based generative adversarial networks (GANs). Park et al. showed that a data is typically multi-modal, and it is necessary to separate modes and assign a generator to each mode of data, e.g., one generator for long-hair female, another generator for short-hair male and so on for a GAN generating facial images~\cite{Park2018}. In our case, we try to separate the two modes, i.e., linear and non-linear characteristics, of the user-item interaction bipartite graph.

==> algorithm_hmlet_end.tex <==
% \begin{algorithm}[t]
% % \small
% \footnotesize
% \caption{\oure }
% \label{algo:type_d} 
%   \begin{flushleft}
%       \textbf{Input:} user embedding $u_0$, item embedding $v_0$, linear layer $k$ and non-linear layer $k\prime$ \\
%       \textbf{Output:} residual $\hat{r}$, which will be used in the final prediction
%   \end{flushleft}
%     \begin{algorithmic}[1]
%         \STATE $e_u^{L_0^l}, e_u^{L_0^n} \leftarrow e_u $ \hfill \Comment{initial user embedding}
%         \STATE $e_v^{L_0^l}, e_v^{L_0^n} \leftarrow e_v $ \hfill \Comment{initial item embedding}

%         \REPEAT
%             \FOR{$i \leftarrow 1 \; \text{to} \; k$}
%                 \IF{$i \le (k-k\prime)$}
%                 \STATE $e_u^{L_{(i)}^l}, e_v^{L_{(i)}^l}  \leftarrow \test{AGG} (e_u^{L_{(i-1)}^l}, e_v^{L_{(i-1)}^l} )$
%                 \STATE $\hat{r} \mathrel{{+}{=}} e_u^{L_{(i)}^l} \odot\  e_v^{L_{(i)}^l}$

%                 \ELSIF{$i > (k-k\prime)$}
%                 \STATE $e_u^{L_{(i+k\prime)}^l} , e_v^{L_{(i+k\prime)}^l} \leftarrow \text{AGG}(e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l})$
%                 \STATE $e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n} \leftarrow \text{AGG}(e_u^{L_{(i-k\prime-1)}^n}, e_v^{L_{(i+k\prime-1)}^n})$
%                 % \STATE $e^{L^l} \leftarrow e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}$
%                 % \STATE $e^{L^n} \leftarrow e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n}$
%                 % \STATE $e^{L^g} \leftarrow GN(e^{L^l}, e^{L^n})$ \hfill \Comment{gating network phase}
%                 % \STATE $g \leftarrow GN(e^{L^l}, e^{L^n})$ \hfill \Comment{gating network phase}
%                 \STATE $g \leftarrow GN\left( (e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}), (e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n}) \right) $ \hfill \Comment{eq.(9)}
%                 % \STATE $e^{L^g} \leftarrow g \odot \text{stack}(e^{L^l}, e^{L^n})$
%                 \STATE $e_u^{L_{i-k\prime}^g}, e_v^{L_{i-k\prime}^g} \leftarrow g \odot \text{stack}\left( (e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}), (e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n}) \right)$
%                 % \STATE $e_u^{L_{i-k\prime}^g}, e_v^{L_{i-k\prime}^g} \leftarrow e^{L^g}$
%                 \STATE $\hat{r} \mathrel{{+}{=}} e_u^{L_{i-k\prime}^g} \odot\ e_v^{L_{i-k\prime}^g}$
%                 \ENDIF
%             \ENDFOR
%         \UNTIL{converge}
%     \end{algorithmic}
% \end{algorithm}
\SetInd{0.2em}{0.2em}
\begin{algorithm}[t]
% \footnotesize
\small
\SetAlgoLined
\DontPrintSemicolon
    Initialize $e_u^{L_0^l}, e_u^{L_0^n}, e_v^{L_0^l}, e_v^{L_0^n},$  linear layer $k$ and non-linear layer $k\prime$\;
    % $e_u^{L_0^l}, e_u^{L_0^n} \leftarrow e_u $ \;
    % $e_v^{L_0^l}, e_v^{L_0^n} \leftarrow e_v $ \;
    \While {the BPR loss $L$ is not converged}{
    \For{$i \leftarrow 1 \; \text{to} \; k$}{ 
        \uIf{$i \le (k-k\prime)$}{
            $e_u^{L_{(i)}^l}, e_v^{L_{(i)}^l} = \test{AGG} (e_u^{L_{(i-1)}^l}, e_v^{L_{(i-1)}^l} )$ \;
            $\hat{r} \mathrel{{+}{=}} e_u^{L_{(i)}^l}  \odot\  e_v^{L_{(i)}^l}$ \;
            
          }
          \Else{
             $e_u^{L_{(i+k\prime)}^l} , e_v^{L_{(i+k\prime)}^l} = \text{AGG}(e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l})$ \;
             $e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n} = \text{AGG}(e_u^{L_{(i-k\prime-1)}^n}, e_v^{L_{(i+k\prime-1)}^n})$ \;
             $g =$ \text{GN}$\big( e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}, e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n}  \big) $ \;
             $e_u^{L_{i-k\prime}^g}, e_v^{L_{i-k\prime}^g} = g \cdot \text{stack}\big( e_u^{L_{(i+k\prime)}^l}, e_v^{L_{(i+k\prime)}^l}, e_u^{L_{(i-k\prime)}^n} , e_v^{L_{(i-k\prime)}^n} \big)$ \;
             $\hat{r} \mathrel{{+}{=}} e_u^{L_{i-k\prime}^g} \odot e_v^{L_{i-k\prime}^g}$ \;
          }
    }
    \Return $\hat{r}$ \;
}
\textbf{end}
\caption{\oure}
\label{algo:type_d} 
\end{algorithm}

==> fig-degree-distribution.tex <==
\begin{figure}[t]
\centering
\begin{tikzpicture}
\begin{axis}[
width=5cm,
% height=5cm, 
ylabel=Degree, xlabel=Nodes,
ymin=0, ymax=400,
nodes near coords align=vertical,
legend columns=3,
% legend pos=outer north,
legend cell align=left,
legend style={at={(0.50,1.2)},font=\footnotesize, anchor=center},
]
% FNL
\addplot[color=blue,mark=triangle,] file {results/FNL-degree.txt};\addlegendentry{FNL}
% PNL
\addplot[color=red,mark=oplus,] file {results/PNL-degree.txt};\addlegendentry{PNL}
% FL
\addplot[color=black,mark=square,] file {results/FL-degree.txt};\addlegendentry{FL}
% EAT
\end{axis}
\end{tikzpicture}
\vspace{-0.3cm}
\caption{Degree distribution on Gowalla.}\label{fig:degree}
\vspace{-0.3cm}
\end{figure}

==> fig-rq2.tex <==
\begin{figure*}[t!]
\centering
\begin{tikzpicture}
\centering
\small
\begin{customlegend}[legend columns=4,legend style={align=center,draw=none,column sep=1.5ex}, legend cell align={left},
  legend entries={{\Etype}, {\Btype}, {\Ftype}, {\Dtype}}]
  \addlegendimage{area legend, draw=black, fill=black} %, postaction={pattern=grid}
  \addlegendimage{area legend, draw=black, fill=black!70} %, postaction={pattern=horizontal lines}
  \addlegendimage{area legend, draw=black, fill=black!40} %, postaction={pattern=vertical lines}
  \addlegendimage{area legend, draw=black, fill=black!10} %, postaction={pattern=dots}
  \end{customlegend}
\end{tikzpicture}

\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\amazon}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.0250, ymax=0.0300,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@20},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small },
        scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3},% rotate=20, 
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.0280)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.0280)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.0280)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.0300)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\yelp}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.0390, ymax=0.0440,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@20},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small }
        scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3}, % rotate=20, 
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.0431)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.0430)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.0430)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.0434)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\go}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.1190, ymax=0.1240,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@20},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small }, % rotate=20, 
       scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3},
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.1221)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.1221)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.1219)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.1231)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\vspace{-0.25cm}
\caption{Comparison ndcg (K=20) with all types of {\ours} on three public benchmarks.}
\label{fig:comparison-rq1}
\vspace{-0.25cm}
\label{fig:rq2}
\end{figure*}

\begin{figure*}[t!]
\centering
\begin{tikzpicture}
\centering
\small
\begin{customlegend}[legend columns=4,legend style={align=center,draw=none,column sep=1.5ex}, legend cell align={left},
  legend entries={{\Etype}, {\Btype}, {\Ftype}, {\Dtype}}]
  \addlegendimage{area legend, draw=black, fill=black} %, postaction={pattern=grid}
  \addlegendimage{area legend, draw=black, fill=black!70} %, postaction={pattern=horizontal lines}
  \addlegendimage{area legend, draw=black, fill=black!40} %, postaction={pattern=vertical lines}
  \addlegendimage{area legend, draw=black, fill=black!10} %, postaction={pattern=dots}
  \end{customlegend}
\end{tikzpicture}

\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\amazon}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.018, ymax=0.023,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@10},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small },
        scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3},% rotate=20, 
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.0209)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.0208)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.0208)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.0223)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\yelp}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.0290, ymax=0.0340,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@10},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small }
        scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3}, % rotate=20, 
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.0330)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.0328)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.0330)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.0332)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\begin{tabular}{c}  
\begin{tikzpicture}
  \centering
  \begin{axis}[
        ybar=7pt, 
        height=3cm, width=.5\textwidth,
        bar width=8.5pt,
        % bar shift=2pt,
        title={\textbf{\go}},
        x=1.5cm,
        ymajorgrids=true, 
        tick align=inside,
        major grid style={line width=.2pt,draw=white},
        % enlarge y limits={value=.1,upper},
        enlarge x limits=0.15,
        ymin=0.1020, ymax=0.1060,
        axis x line*=center,
        axis y line*=left,
        ylabel={NDCG@10},
        % xlabel={Types},
        symbolic x coords={Types},
        xtick=data,
        nodes near coords align=vertical,
        clip=false,
        % xticklabel style={font=\small }, % rotate=20, 
       scaled y ticks = false,
        y tick label style={/pgf/number format/fixed,
         /pgf/number format/precision=3},
    ]
    % GEE-A
    \addplot [draw=black, fill=black] coordinates {
      (Types, 0.1046)};
    % GEE-F
    \addplot [draw=black, fill=black!70] coordinates {
      (Types, 0.1042)};
    % GEE-M
    \addplot [draw=black, fill=black!40] coordinates {
      (Types, 0.1043)};
    % GEE-E
    \addplot [draw=black, fill=black!10] coordinates {
      (Types, 0.1052)};
  \end{axis}
\end{tikzpicture}
\end{tabular}
\vspace{-0.25cm}
\caption{Comparison ndcg (K=10) with all types of {\ours} on three public benchmarks.}
\label{fig:comparison-rq2}
\vspace{-0.25cm}
\label{fig:rq2}
\end{figure*}

==> macros.tex <==

\newcommand{\ie}{{\it i.e.,}}
\newcommand{\eg}{{\it e.g.,}}
\newcommand{\yc}[1]{\textcolor{blue}{#1}}
\newcommand{\js}[1]{\textcolor{green}{#1}}
\newcommand{\note}[1]{\textcolor{red}{#1}}
\newcommand{\go}{Gowalla}
\newcommand{\yelp}{Yelp2018}
\newcommand{\amazon}{Amazon-Book}
\newcommand{\light}{LightGCN}
\newcommand{\lrgccf}{LR-GCCF}
\newcommand{\ngcf}{NGCF}
\newcommand{\Etype}{\textsc{\textsf{HMLET}}(All)}
\newcommand{\Btype}{\textsc{\textsf{HMLET}}(Front)}
\newcommand{\Ftype}{\textsc{\textsf{HMLET}}(Middle)}
\newcommand{\Dtype}{\textsc{\textsf{HMLET}}(End)}

\newcommand{\ourf}{\textsc{\textsf{HMLET}}(Front)}
\newcommand{\ourm}{\textsc{\textsf{HMLET}}(Middle)}
\newcommand{\oure}{\textsc{\textsf{HMLET}}(End)}

\newcommand{\ours}{\textsc{\textsf{HMLET}}}
\newcommand{\geee}{\textsc{\textsf{GEE-E}}}

==> sec-analysis.tex <==
\subsection{In-Detail Analysis}\label{sec:analysis}
In this subsection, we analyze in detail class ratio and the characteristics of each node selected by gating networks to confirm factors of determining which embedding propagation is effective. In order to analyze accurately, we utilize the results of {\Dtype} with the best accuracy among the all types of {\ours}.

\subsubsection {\bfseries{Node class and graph centrality}}\label{sec:node_class}
We first classify all nodes into three classes according to the type of the embedding selected by gating networks:

\begin{itemize}[leftmargin=*]
    \item {\bfseries Full-Non-Linearity (FNL)} is a class of nodes in which all embeddings selected by the gating networks are non-linear embeddings.

\item {\bfseries Partial-Non-Linearity (PNL)} is a class of nodes in which the embeddings selected by the gating networks are mixed with linear embeddings and non-linear embeddings.

\item {\bfseries Full-Linearity (FL)} is a class of nodes in which all embeddings selected by the gating networks are linear embeddings.
\end{itemize}

We next introduce three graph centrality measures
to clarify distinct characteristics of nodes that determine linear/non-linear embedding propagation:

\begin{itemize}[leftmargin=*]

\item {\bfseries Page Rank} 
~\cite{page1999pagerank} measures the relative importance of a node in the network. The more nodes with high rank are linked the more important node.

\item {\bfseries Betweenness Centrality} ~\cite{brandes2001centralitybet} measures the centrality of a node as an intermediary in the network. The more the node is included within the shortest path between all pairs of nodes in the network, the higher the betweenness centrality.

\item {\bfseries Closeness Centrality}~\cite{freeman1978centralitycls}
measures the centrality of a node by considering not only the direct connection information of the node but also the indirect connection information in the network. The more nodes are linked directly/indirectly the higher the closeness centrality.
\end{itemize}

\subsubsection {\bfseries{Analyzing relation of effectiveness to class ratio (RQ3)}}\label{sec:node_class_ratio}Table \ref{tab:class ratio} shows the class ratio of nodes on three datasets. Specifically, in the {\amazon} and {\yelp} datasets, most nodes were classified as FNL and PNL (about 47-8\%, 50-2\%), and very a few nodes were classified as FL (about 2\%). However, in the {\go} dataset, the ratio of FL nodes is about 12\%, which is relatively quite high compared to the other two datasets.

From the recommendation evaluation results in Table \ref{tab:comparison-rq1}, \ref{tab:comparison-rq2}  we found that the higher the ratio of FNL nodes, the better {\ours} methods perform than the linear GCN, LightGCN which shows the best performance among baselines. The results of analysis explain why remarkable performance improvements is observed in the Amazon dataset. Since the {\amazon} has the smallest FL node ratio, and the FNL ratios are high, the effectiveness is significantly improved when using non-linear embedding propagation together.

\subsubsection {\bfseries{Analyzing characteristics of class-specific nodes (RQ4).}}

We certainly confirm with previous experimental results that the linear/non-linear characteristics can be appropriately selected, although its ratio is changed depending on the dataset. We next analyze node attributes that determines which embedding is effective and use it to give insight for selection between linear embedding propagation and non-linear embedding propagation. 

Figure~\ref{fig:node_degree_distribution} shows the result of a degree distribution of nodes in the Amazon-Book dataset.\footnote{The other two datasets also show a similar trend, but due to page limit, only the result of the Amazon-Book dataset is shown here.} The x-axis represents nodes percentage ascending by degree at 10\% intervals, and the y-axis represents class ratio.
Figure~\ref{fig:box_plot} represents the graph centrality of the class-specific nodes in the {\amazon} dataset as a boxplot. From Figure~\ref{fig:node_degree_distribution} and Figure~\ref{fig:box_plot}, it can be seen that the degree and all centralities increase in the order of the FL, PNL, and FNL node in general. Here, we analyze the meaning of the above results for each class.

\begin{itemize}[leftmargin=*]
\item {\bfseries Full Non-Linearity (FNL) Nodes Attribute} 
 This node is either an active user or popular item with more direct/indirect interaction information (i.e., high degree and closeness centrality) and a high influence (i.e., high page rank and betweenness centrality) than nodes of other classes. They have a lot of direct/indirect interactions with other nodes and a strong influence, so they will receive a lot of information in the process of embedding propagation. However, since there is a lot of information being received, more informative and less informative nodes can coexist in predicting or presenting user preference. Therefore, it would be necessary to accurately distinguish nodes that are more informative to each of them through a non-linear operation.
 \item {\bfseries Full Linearity (FL) Nodes Attribute}
 This node is either a user or item that does not have much direct/indirect interaction information (i.e., low degree and closeness centrality) and a little influence (i.e., low page rank and betweenness centrality) compared to nodes of other classes. They do not have many direct/indirect interactions with other nodes and little influence, so the information they receive may mostly consist of information informative to them. Therefore, a simple linear operation (e.g., average) without a non-linear operation will be enough to well predict or represent the user's preference.
 \item {\bfseries Partial Non-Linearity (PNL) Nodes Attribute}
 This node, compared to nodes of other classes, is a user or item with neither too large nor too small direct/indirect interaction information (i.e., degree and closeness centrality between nodes in different classes) and influence (i.e., page rank and betweenness centrality between nodes in different classes). In other words, although they have many direct neighbors, there are few indirect neighbors connected to direct neighbors (because direct neighbors are mainly FL nodes), or even if there are few direct neighbors, their indirect neighbors could be many (because direct neighbors are mainly FNL nodes). Therefore, they need to perform non-linear or simple linear operations according to the information they receive from direct/indirect interactions during the process of embedding propagation.
\end{itemize}
 
 
 \begin{figure*}[t!]
\centering
% \usepackage{pgfplots}
\pgfplotsset{compat=1.8}
\usepgfplotslibrary{statistics}
\begin{subfigure}
\begin{tikzpicture}[scale=0.7]
  \begin{axis}[
    % [
    xlabel = {Page Rank},
    boxplot/draw direction=y,
    xtick={1,2,3},
    xticklabels={FNL, PNL, FL},
    x tick label style={font=\footnotesize, text width=2.5cm, align=center}
    ]
    \addplot+[
    boxplot prepared={
      lower whisker=1.18196E-06,
      lower quartile=3.3164E-06,
      median=4.8673E-06,
      upper quartile=8.05604E-06,
      upper whisker=1.51649E-05,
            %  average=8.0014E-06
    }, color = black, fill=black!60
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=1.16982E-06,
      lower quartile=3.14872E-06,
      median=4.54145E-06,
    %   average=6.02811E-06,
      upper quartile=6.63666E-06,
      upper whisker=1.18678E-05
    }, color = black, fill=black!40
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=1.21219E-06,
      lower quartile=2.68252E-06,
      median=3.61638E-06,
      upper quartile=5.16359E-06,
      upper whisker=8.87023E-06,
    %   average=4.76206E-06
    }, color = black, fill=black!20
    ] coordinates{};
    \end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}
\begin{tikzpicture}[scale=0.7]
  \begin{axis}[
    % [
    xlabel = {Betweenness Centrality},
    boxplot/draw direction=y,
    xtick={1,2,3},
    xticklabels={FNL, PNL, FL},
    x tick label style={font=\footnotesize, text width=2.5cm, align=center}
    ]
    \addplot+[
    boxplot prepared={
      lower whisker=0,
      lower quartile=1.5827E-06,
      median=4.66162E-06,
      upper quartile=1.51682E-05,
      upper whisker=3.55464E-05,
            %  average=3.04861E-05
    }, color = black, fill=black!60
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=0,
      lower quartile=1.28016E-06,
      median=3.50505E-06,
    %   average=1.31815E-05,
      upper quartile=9.67357E-06,
      upper whisker=2.22579E-05
    }, color = black, fill=black!40
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=0,
      lower quartile=6.21681E-07,
      median=1.83557E-06,
      upper quartile=5.4101E-06,
      upper whisker=1.24468E-05,
    %   average=7.84346E-06
    }, color = black, fill=black!20
    ] coordinates{};
    \end{axis}
\end{tikzpicture}
\end{subfigure}
\begin{subfigure}
\begin{tikzpicture}[scale=0.7]
  \begin{axis}[
    % [ylabel = {Closeness Centrality},
    xlabel ={Closeness Centrality},
    boxplot/draw direction=y,
    xtick={1,2,3},
    xticklabels={FNL, PNL, FL},
    x tick label style={font=\footnotesize, text width=2.5cm, align=center}
    ]
    \addplot+[
    boxplot prepared={
      lower whisker=0.206843691,
      lower quartile=0.239632048,
      median=0.24964174,
      upper quartile=0.261528364,
      upper whisker=0.294344759,
            %  average=0.250870241
    }, color = black, fill=black!60
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=0.205991771,
      lower quartile=0.235977482,
      median=0.245726143,
    %   average=0.245588375,
      upper quartile=0.255969292,
      upper whisker=0.285935459
    }, color = black, fill=black!40
    ] coordinates{};
    \addplot+[
    boxplot prepared={
      lower whisker=0.15967715,
      lower quartile=0.21024025,
      median=0.230146713,
      upper quartile=0.244418274,
      upper whisker=0.295508604,
    %   average=0.227881812
    }, color = black, fill=black!20
    ] coordinates{};
    \end{axis}
\end{tikzpicture}
\end{subfigure}
\caption{Boxplots about centralities in Amazon-Book dataset. The Yelp2018 dataset shows a similar trend, but in the Gowalla dataset, the results of FL nodes are similar to the results of PNL nodes in the page rank and betweenness centrality.}
\label{fig:box_plot}
\end{figure*}

To make sure our interpretation is correct, we show the tendency of neighbors per each class. So, we calculate the similarity (i.e., cosine similarity) between the class-specific node and its direct neighbors using embeddings learned by {\Dtype}.
As can be seen from Table \ref{tab:similarity}, the mean of the similarity between class-specific nodes and their neighbors increases in the order of FNL, PNL, and FL node, and the variance increases in the order of FL, PNL, and FNL node.

From these results, we can confirm that FNL nodes' neighbors variously are consist of the more informative and less informative nodes (i.e., relatively low similarity means and high similarity variance) and FL nodes' neighbors mainly consist of informative nodes (i.e., high similarity mean and low similarity variance), and PNL nodes' neighbors have the characteristics of the FNL node and the FL node evenly (i.e., similarity mean and variance between nodes in different classes).

In this section, through multiple measures and experiments, we analyzed the characteristics of each of the user-item interactions that gating networks select linear or non-linear embedding propagation about. To the best of our knowledge, this is the first study to find out that linear and non-linear features in user-item interactions can coexist, and analyze what type of node each feature can occur in.

\begin{figure}
\centering
\begin{tikzpicture}[scale=0.7]
\begin{axis}[
    xlabel={Nodes ascending  by degree (at 10\% intervals)},
    % ylabel={Class-specific node ratio},
    % xlabel={Degree in ascending order (at 10\% intervals)},
    ylabel={Class ratio},
    xmin=0, xmax=90,
    ymin=0, ymax=80,
    xtick={0,10,20,30,40,50,60,70,80,90},
    xticklabels={10\%, 20\%, 30\%, 40\%, 50\%, 60\%, 70\%, 80\%, 90\%, 100\%,},
    ytick={0,10,20,30,40,50,60,70,80},
    legend pos=north west,
    ymajorgrids=true,
    grid style=dashed,
    mark options={solid}
]
\addplot[
   mark=*
    ]
    coordinates {
    (90,78.11895919) (80,75.20940871)
		(70,62.10739659) (60,54.9429539) (50,48.86218309) (40,42.92219384)
		(30,38.13066353) (20,34.57854787) (10,29.58106313) (0,24.81291262)
    };
\addplot[
    dashed,mark=triangle*
    ]
    coordinates {
    (90,11.70514673) (80,21.1389107)
		(70,31.2421691) (60,34.72602399) (50,35.97356713) (40,37.39357856)
		(30,37.8853709) (20,38.7649476) (10,37.60506112) (0,28.32400165)
    };
\addplot[
    dashed,mark=square*
    ]
    coordinates {
    (90,10.17589408) (80,3.651680582)
		(70,6.65043431) (60,10.33102211) (50,15.16424978) (40,19.68422761)
		(30,23.98396556) (20,26.65650453) (10,32.81387575) (0,46.86308574)
    };
    \legend{FNL,PNL,FL}
\end{axis}
\end{tikzpicture}
\caption{Node distributions in each class.}
\label{fig:node_degree_distribution}
\end{figure}



\begin{table}
  \caption{Similarity between the class-specific node and its direct neighbors}
  \label{tab:similarity}
  \begin{tabular}{cccc}
    \toprule
    Similarity & FNL & PNL & FL \\
    \midrule
    Mean & 0.6369 & 0.6449 & 0.7157 \\
    Variance & 0.0179 & 0.0162 & 0.0160 \\
  \bottomrule
\end{tabular}
\end{table}



\subsubsection{{\bfseries 

==> sec-conclusions.tex <==
\section{Conclusions and Future Work}
In GCN-based recommender, we analyzed which linear/non-linear embedding propagation is appropriate and the characteristics of each embedding propagation systems by focusing on the existing GCN’s issues related to the use of linear embedding and non-linear embedding. Our proposed recommender system HEMLET can hybridize the linear and non-linear embedding propagation through the gating network in each layer by dynamically selecting appropriate embedding propagation. Our method shows the best accuracy in all datasets and we also presented in-depth analysis how linearity and non-linearity of nodes are decided in a network. Moreover, we classify users/items into three classes (Full-Linearity, Full-Non-Linearity, and Partial-Non-Linearity) depending on our gating network’s selections and find correlations between nodes’ centralities and their characteristics. We hope that our discovery encourages much follow-up research work.
\label{sec:conclusions}

==> sec-evaluation.tex <==
\section{Experiments}\label{sec:experiments}

In this section, we evaluate our proposed approach via extensive experiments. We designed the experiments, aiming at answering the following key research questions (RQs):

{\begin{itemize}[leftmargin=*]
\item {\bfseries RQ1:} Does hybridizing the linear/non-linear embedding propagation provide more-accurate recommendations than either only using linear embedding or non-linear embedding?
\item {\bfseries RQ2:} 
Which architecture of our gating network is most effective in terms of recommendation accuracy?
\item {\bfseries RQ3:} 
How each embedding propagation affects to recommendation accuracy?
%\item {\bfseries RQ3:} 
%How embedding propagation ratio affects recommendation accuracy?
\item {\bfseries RQ4:} 
What are the characteristics of the nodes that affects to determination to use linear/non-linear embedding propagation?
\end{itemize}}

\begin{table}
  \caption{Statistics of public benchmark dataset}
  \label{tab:datasets}
  \begin{tabular}{ccccl}
    \toprule
    \textbf{Dataset} & \textbf{User \#} & \textbf{Item \#} & \textbf{Interaction} \# & \textbf{Sparsity} \\
    \midrule
    \textbf{\go} & 29,858 & 40,981 & 1,027,370 & 99.916\%\\
    \textbf{\yelp} & 31,668 & 38,048 & 1,561,406 & 99.870\%\\
    \textbf{\amazon} & 52,643 & 91,599 & 2,984,108 & 99.938\%\\
  \bottomrule
\end{tabular}
\end{table}

\begin{table*}[]
\caption{Comparison overall performance (K=20) with baseline models on three public benchmarks}
\label{tab:comparison-rq1}
\begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
\toprule
Dataset  & \multicolumn{3}{c|}{Amazon-Book}                                                                                                                                                                       & \multicolumn{3}{c|}{Yelp2018}                                                                                                                                                                         & \multicolumn{3}{c|}{Gowalla}                                                                                                                                                                          \\ \hline
Metrics   & NDCG                                                       & Recall                                                     & Precision                                                  & NDCG                                                       & Recall                                                     & Precision                                                  & NDCG                                                       & Recall                                                     & Precision\\                  \hline\hline BPR      & 0.0181                                                              & 0.0307                                                              & 0.0065                                                              & 0.0289                                                              & 0.0476                                                              & 0.0062                                                              & 0.0847                                                              & 0.1341                                                              & 0.0203                                                              \\ \hline
WRMF     & 0.0242                                                            & 0.0405                                                            & 0.0085                                                            & 0.0402                                                              & 0.0645                                                              & 0.0145                                                              & 0.1007                                                              & 0.1538                                                              & 0.0243        \\ \hline
NGCF     & 0.0250                                                            & 0.0426                                                            & 0.0086                                                              & 0.0371                                                            & 0.0601                                                            & 0.0134                                                            & 0.1071                                                            & 0.1661                                                            & 0.0253                                                            \\ \hline
LR-GCCF  &  0.0213                                                           & 0.0361                                                            & 0.0077                                                            & 0.0351                                                            & 0.0581                                                            & 0.0129                                                            & 0.0989                                                            & 0.1545                                                            & 0.0240                                                           \\ \hline
{\light} & \textit{0.0283}                                                              & \textit{0.0484}                                                             & \textit{0.0099}                                                              & \textit{0.0420}                                                              & \textit{0.0678}                                                              & \textit{0.0152}                                                              & \textit{0.1212}                                                              & \textit{0.1870}                                                              & \textit{0.0288}                                                              \\ \hline\hline

\textbf{{\ours}}    & \textbf{\begin{tabular}[c]{@{}c@{}}0.0300\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0510\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0103\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0434\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0696\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0155\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.1231\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.1908\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0293\end{tabular}} \\ \hline 
\%Improv.      & 6.00\%                                                              & 5.37\%                                                              & 4.04\%                                                              & 3.33\%                                                              & 2.65\%                                                              & 1.97\%                                                              & 1.56\%                                                              & 2.03\%                                                             & 1.73\%                                                             \\ \hline
p-value     & 1.59E-37
                                                            & 1.71E-34
                                                            & 5.16E-36
                                                            &  5.57E-58
                                                             & 2.90E-39


                                                              & 1.61E-44
                                                              & 8.51E-25                                                              & 4.17E-131                                                              & 3.39E-27                      \\

\bottomrule\hline
\end{tabular}
\end{table*}

 \begin{table*}[]
 \caption{Comparison overall performance (K=10) with baseline models on three public benchmarks}
 \label{tab:comparison-rq2}
 \begin{tabular}{|c|c|c|c|c|c|c|c|c|c|}
 \toprule
 Dataset  & \multicolumn{3}{c|}{Amazon-Book}                                                                                                                                                                       & \multicolumn{3}{c|}{Yelp2018}                                                                                                                                                                         & \multicolumn{3}{c|}{Gowalla}                                                                                                                                                                          \\ \hline
 Metrics   & NDCG                                                       & Recall                                                     & Precision                                                  & NDCG                                                       & Recall                                                     & Precision                                                  & NDCG                                                       & Recall                                                     & Precision\\                  \hline\hline BPR      & 0.0133                                                               & 0.0176                                                              & 0.0073                                                              & 0.0216                                                              & 0.0277                                                              & 0.0071                                                              & 0.0715                                                             & 0.0926                                                              & 0.0274                                                              \\ \hline
 WRMF     & 0.0181                                                            & 0.0236                                                            & 0.0097                                                            & 0.0308                                                              & 0.0386                                                              & 0.0170                                                              & 0.0864                                                              & 0.1084                                                              & 0.0336       \\ \hline
 NGCF     & 0.0186                                                          & 0.0250                                                            & 0.0099                                                           & 0.0280                                                            & 0.0350                                                            & 0.0155                                                            & 0.0916                                                            & 0.1162                                                            & 0.0351                                                             \\ \hline
 LR-GCCF  &  0.0158                                                           & 0.0215                                                            & 0.0087                                                            & 0.0264                                                            & 0.0349                                                            & 0.0150                                                            &  0.0841                                                            & 0.1081                                                           & 0.0327                                                          \\ \hline
 {\light} & \textit{0.0209}                                                             & \textit{0.0278}                                                             & \textit{0.0112}                                                              & \textit{0.0321}                                                              & \textit{0.0404}                                                              & \textit{0.0180}                                                              & \textit{0.1040}                                                              & \textit{0.1314}                                                             & \textit{0.0399}                                                              \\ \hline\hline

 \textbf{{\ours}}    & \textbf{\begin{tabular}[c]{@{}c@{}}0.0223\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0298\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0118\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0332\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0414\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0183\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.1052\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.1329\end{tabular}} & \textbf{\begin{tabular}[c]{@{}c@{}}0.0404\end{tabular}} \\ \hline 
 \%Improv.      & 6.27\%                                                              & 7.19\%                                                              & 5.35\%                                                              & 3.42\%                                                              & 2.41\%                                                              & 1.66\%                                                              & 1.15\%                                                              & 1.14\%                                                             & 1.25\%                                                             \\ \hline
 p-value     & 1.09E-39                                                             & 1.32E-38

                                                             &  4.72E-37                                                           & 1.31E-42
                                                               & 1.06E-30
                                                               & 1.44E-32                                                               & 7.83E-22                                                              & 9.79E-21                                                              & 1.21E-18
                       \\

 \bottomrule\hline
 \end{tabular}
 \end{table*}

\subsection{Experimental Setup}
\subsubsection{\bfseries{Datasets}}
For evaluation, we used three real-word datasets: \go, \yelp, and \amazon\ from various domains. They are all publicly available. Table~\ref{tab:datasets} shows the detailed statistics of the three datasets.

\begin{itemize}[leftmargin=*]
\item \textbf{\go} is a location-based social networking website where users share their locations by checking-in~\cite{liang2016modeling}. This dataset contains user-website interactions.

\item  \textbf{\yelp} is subset of small businesses and user data used in Yelp Dataset Challenge 2018. %\footnote{https://www.yelp.com/dataset/download}.
This dataset contains user-business interactions.

\item  \textbf{\amazon} is huge purchase history of Amazon users. {\amazon} has highest sparsity among these three public data sets. This dataset contains user-item interactions.
\end{itemize}

Following~\cite{Wang19NGCF}, we filtered out those users and items with less than ten interactions in all datasets (\ie\ a 10-core setting). For testing, we then split a dataset into training (80\%), validation (10\%), and test (10\%) sets in the same way as in ~\cite{Wang19NGCF}.


\subsubsection{\bfseries{Competing Methods}}
We compare the {\ours} with  2 baselines and 3 state-of-the-arts GCN-based models to verify its effectiveness.%\footnote{We performed the same as the experimental setup in~\cite{He20LightGCN}; thus, we did not compare with other neural network based methods that showed the lower accuracy than \light.}%
As the baselines, we compare ours with the traditional MF-based models:
\begin{itemize}[leftmargin=*]
    \item \textbf{WRMF}~\cite{Hu08WRMF} is a matrix factorization (MF) optimized by the \textit{weight alternating least square} (WALS) technique. It aims to minimize the errors between the real and predicted rating scores.
    \item  \textbf{BPRMF}~\cite{Rendle09BPR} is an MF optimized by the \textit{Bayesian personalized ranking} (BPR) loss. It aims to maximize the relative preference differences between a single item rated by a user and another single item that she has not rated.
\end{itemize}

Also, we compare ours with a state-of-the-art non-linear GCN and two liner GCNs:
\begin{itemize}[leftmargin=*]
    \item \textbf{\ngcf}~\cite{Wang19NGCF} is a non-linear GCN-based recommender system performing residual prediction.
    \item  \textbf{\lrgccf}~\cite{Chen20LRGCCF} is a linear GCN-based recommender system performing residual prediction.
    \item  \textbf{\light}~\cite{He20LightGCN} is a linear GCN-based recommender system performing residual prediction. This method differs from the LR-GCCF in that it removes all redundant parameters.
\end{itemize}

For MF-based methods, we used the implementations in the popular open-source NeuRec.%\footnote{https://github.com/wubinzzu/NeuRec}%
For GCN-based methods, we used the source codes provided by the authors~\cite{He20LightGCN,Chen20LRGCCF,Wang19NGCF}.
% % \subsubsection {\bfseries{Evaluation Metrics}}
% % \vspace{1mm}
% \note{(position?)\noindent\textbf{Evaluation Metrics.}
To evaluate the accuracy of \ours\ and the competing methods, we performed top-$k$ (20, 10)  recommendation using each method and measured its accuracy in terms of Precision, Recall, and \textit{normalized discounted cumulative gain} (NDCG), which are popularly used in a recommendation research~\cite{Wang19NGCF,Chen20LRGCCF,He20LightGCN}.

\subsubsection{\bfseries{Hyper-parameter Settings}}
For parameter tuning, we found the best settings in {\ours} and competing methods via extensive grid search with the validation set. The best setting found in {\ours} as follows: the number of the layer for linear GCN = 4, the number of the layer for non-linear GCN = 4({\Etype}) and 2({\Dtype}, {\Btype}, {\Ftype}), optimizer = Adam, learning rate $=0.001$, L2 regularization coefficient $\lambda = 1e-4$, mini-batch size $=2,048$, dropout rate $=0.4$. Also, for a fair comparison, we set embedding size for all GCN-based methods to the same dimensionality, $512$. In non-linear GCN, we use two nonlinear activation functions: Leaky-ReLU (negative slope = 0.01) and ELU ($\alpha$ = 1.0). We set temperature of Straight-Through Gumbel-Softmax~\cite{jang16categorical} for decay, original temperature as 0.7, minimum temperature as 0.01, and temperature decay value as 0.005.

\subsection{Performance Comparison}
% We first compare best type of {\ours} (\geee) with baseline models. Also, we compare each type of {\ours} to search most effective structure of proposed models.

\subsubsection{\bfseries{Comparison with competing methods (RQ1)}} \label{sec:comparison_competing_methods}
We conducted comparative experiments to show greater accuracy of {\ours} than that of 5 competing methods, \ie WRMF, BPRMF, NGCF, LRGCCF, and LightGCN.
Tables~\ref{tab:comparison-rq1} and ~\ref{tab:comparison-rq2} illustrate the result.
%\footnote{Due to space limitations, we omit the results for other top-$k$, which showed tendency similar to those in Tables~\ref{tab:comparison-rq1} and ~\ref{tab:comparison-rq2}. Please refer to all the results in [web link].} 
In Tables~\ref{tab:comparison-rq1} and ~\ref{tab:comparison-rq2}, the value in \textit{boldface} indicates the best accuracy in each column, and the value in \textit{italic} does the accuracy obtained from the best performer among all `competing' methods. 
Also, `\% Improve' indicates the degree of accuracy improvements from the best competing methods to \ours.
Lastly, we conduct $t$-tests with a 95\% confidence level to verify the accuracy differences between \ours\ and the competing methods.
The results in all measures and all datasets show that all $p$ values (see Tables~\ref{tab:comparison-rq1} and~~\ref{tab:comparison-rq2}) are below $0.05$, indicating the differences are statistically significant.

We summarize the results shown in Tables~\ref{tab:comparison-rq1} and ~\ref{tab:comparison-rq2} as follows. 
First, among five existing methods, we observe that {\light} consistently showed the best accruacy in all datasets. Also, we found that, unlike reported in~\cite{Chen20LRGCCF}, {\ngcf} always outperforms {\lrgccf} in our experiments performed grid search based on our dataset and setting. Second, {\ours} consistently and significantly provides the highest accuracy in all datasets and with all metrics. Specifically, for \amazon/\yelp/\go  \;datasets, {\ours} improve the NDCG@20 of \light, the best performer among the competing methods, by 6.00\%/3.33\%/1.56\%, respectively. Also, for three datasets, {\ours} improve the NDCG@10 of \light, the best performer among the competing methods, by 6.27\%/3.42\%/1.15\%, respectively.

The results indicate that (1) user-item interactions have only linear characteristics but also non-linear characteristics via selection ratio of gating networks as shown in Table~\ref{tab:gating_type} and (2) our gating networks appropriately selects linear/non-linear GCN by considering the inherent properties of users and items. Moreover, exploiting both linear and non-linear GCN is quite effective in predicting users' preferences on items, compared to only using liner GCN (\ie \lrgccf, and \light) or non-linear GCN (\ie \ngcf). We highlight that HMLET shows remarkable improvements in Amazon-Book dataset which is the largest one used in this paper. To discuss our observation, we will perform an in-depth analysis on this phenomenon in Section~\ref{sec:node_class_ratio}
% Similarly, {\ours} also demonstrates its effectiveness exhibiting improvements of Recall and Precision, by 5.37\%/2.65\%/2.03\% and 4.04\%/1.97\%/1.73\%. 
%\yc{Moreover, we highlight that \ours\ shows remarkable improvements in \amazon\ dataset which is the largest one used in this paper. 
%The results represent that as the complexity of user-item interactions increases, \ours\ is more effective. 
%In this sense, we conjecture that the large datasets contain quite a lot of both linearity and non-linearity.
%To demonstrate our claim, we will perform an in-depth analysis on this phenomenon in Section~\ref{sec:analysis}.}
% \note{(insert or not)Our model architecture is designed based on {\light} achieved best performances among existing models by using linear embedding propagation. We next add non-linear aggregating process allocated by gating networks to {\light}.}Our model architecture is consist of linear/non-linear embedding propagation process and gating networks allocating it. In this architecture, demonstration of being superior our model to linearity-based models means that appropriate allocation of linear/non-linear embedding propagation depending on the characteristics of each user-item interaction is more effective more than using only linear one. Moreover, If the decision criteria of allocating linearity and non-linearity will be clarified, we can choose an effective embedding propagation in recommender system, taking into account the characteristics of the data.
\input{fig-rq2}
\subsubsection{\bfseries{Comparison with each model structure (RQ2)}}
As mentioned in Section~\ref{sec:model-prop}, according to location of gating network, we designed four types of gating networks, \ie\ \Etype, \Btype, \Ftype, and \Dtype.
For RQ2, we first compare the accuracices of \ours s equipped with \Etype, \Btype, \Ftype, and \Dtype. Figures~\ref{fig:comparison-rq1} and ~\ref{fig:comparison-rq2} illustrate the result. %\footnote{Due to space limitations, we omit the results for other top-$k$, which showed tendency similar to those in Figures~\ref{fig:comparison-rq1} and ~\ref{fig:comparison-rq2}. Please refer to all the results in [web link].} 
In Figures~\ref{fig:comparison-rq1} and ~\ref{fig:comparison-rq2}, the x-axis represents the all types of {\ours}, and y-axis represents the NDCG@K (10, 20). 

We summarize the results shown in Figures~\ref{fig:comparison-rq1} and ~\ref{fig:comparison-rq2} as follows. First, {\Dtype} types is best performer among all types of {\ours}. Second, The performance of the types except for the {\Dtype} is similar. Specifically, the difference between {\Dtype} and other types is around 1\%/0.5\%/6\%, respectively, on {\go}, {\yelp}, {\amazon}. However, the performance difference of {\Etype}, {\Btype}, {\Ftype}, excluding {\Dtype}, is small as around 0.5\%.

The result indicate that (1) the effectiveness of the gating network depends on layer where the gating network exists, in other words, distance between the target embedding node and the neighboring node and (2) when embedding relationships with relatively long-distance (i.e. layer = 3, 4) neighbor nodes where embedding information can be vanishing due to noise, gating networks can be best utilized via selection of non-liner embedding information of short-distance (i.e. layer = 1, 2) node. As shown in Table~\ref{tab:gating_type}, each type has a 
quite different linear/non-linear embedding selection ratio. Best performer {\Dtype} is that utilization of non-linear embedding is high in layer 3, 4. This observation also applies to the second best-performing {\Etype}. When we perform an extended analysis on a dataset basis, we can observe similar results too. To discuss our observation, we will perform an in-depth analysis on this phenomenon in Section~\ref{sec:node_class_ratio}.

\begin{table*}
  \caption{Selection ratio of embedding propagation each type on {\amazon}}
  \label{tab:gating_type}
  \begin{tabular}{|c|c|c|c|c|c|c|c|c|}
    \toprule
    type of {\ours}&    \multicolumn{2}{c|}{layer 1}&    \multicolumn{2}{c|}{layer 2}&   
    \multicolumn{2}{c|}{layer 3}&   
    \multicolumn{2}{c|}{layer 4}\\   
    \hline
    embedding propagation & Lin. & Non. & Lin. & Non. & Lin. & Non. & Lin. & Non. \\
    \hline
    {\Etype} & 77.05\% & 22.95\% & 60.45\% & 39.55\% & 68.01\% & 31.99\% & 40.77\% & 59.23\% \\
    {\Btype} & 74.3\% & 25.7\% & 62.09\% & 37.91\% & 100\% & 0\% & 100\% & 0\%\\
    {\Ftype} & 100\% & 0\% & 63.03\% & 36.97\% & 72.41\% & 27.59\% & 100\% & 0\%\\
    {\Dtype} &100\% &0\%  &100\%  &0\%  &       5.19\% & 94.81\% & 49.55\% & 50.45\%\\
  \bottomrule
\end{tabular}
\end{table*}

\begin{table}
  \caption{Class ratio of nodes on three datasets}
  \label{tab:class ratio}
  \begin{tabular}{cccc}
    \toprule
    Class & Amazon-Book & Yelp2018 & Gowalla \\
    \midrule
    FNL & 46.78\% & 47.95\% & 27.49\% \\
    PNL & 51.77\% & 49.59\% & 60.84\% \\
    FL & 1.45\% & 2.46\% & 11.67\% \\
  \bottomrule
\end{tabular}
\end{table}

==> sec-intro.tex <==
\section{Introduction}\label{sec:intro}
Recommender system is a personalized information filtering (IF) technology applied to many services, such as E-commerce, advertising, social media, and other many service platforms~\cite{covington2016deep, Ying18pinsage,yuan2020parameter}. The most popular recommender system, Collaborative Filtering (CF), provides personalized preferred items to users by learning user and item embeddings from their historical user-item interactions represented as a bipartite graph, etc ~\cite{8506344,10.1145/3285029,Koren2010,Y.Wu2016,He17NeuMF, Koren09MF,Wang19NGCF,Wang2014,Ebesu2018,Adomavicius2015,Yang2016}. %User-item interactions are represented as a bipartite graph~\cite{Wang19NGCF}.

One of the mainstream research directions in recommender systems is how to learn high-order connectivity of user-item interactions while filtering out noises. Recently, GCN-based CF became popular in recommender systems, because it has strong points to capture latent high-order connectivity between users and items. Since existing GCN is originally designed for graph classification tasks on attributed graph not recommender systems, however, two limitations had been raised out in that approach: training difficulty~\cite{Wu2019SGC,Chen20LRGCCF,He20LightGCN} and over-smoothing~\cite{chen2020measuring, li2018deeper}. Because of sparsity of user-item interactions bipartite graph, non-linear embedding propagation in GCN-based recommender systems generates excessive noise and hinders learning optimal embedding. Also, over-smoothing degrades performance by vanishing the connectivity information. To overcome these problems, usage of linear GCN (GCN based linear embedding propagation) was proposed instead of non-linear GCN (GCN based non-linear embedding propagation)~\cite{Chen20LRGCCF,He20LightGCN}. These methods effectively alleviate the two limitations and produce superior performance over non-linear GCN. Even if, linear GCN was proved for their effectiveness, when only one embedding propagation is used, it is not likely that we properly handle users/items with various characteristics. To us, it is still a question whether linear GCN is really superior to non-linear GCN and if so or not, which factors of graphs decide it.

To this end, we propose a \textbf{H}ybrid \textbf{M}ethod of \textbf{L}inear and non-lin\textbf{E}ar collaborating  fil\textbf{T}ering (\ours), a GCN-based recommender system with dynamically selecting between linear and non-linear embedding propagation considering each user/item's latent characteristics. {\ours} has the following features: i) we adopt a gating concept in each layer to decide between linear GCN and non-linear GCN. ii) we perform residual predictions, which mean embeddings from all layers are aggregated and used together for final predictions. Therefore, we let our gating neural network decide which of linear GCN or non-linear GCN is used for a certain node at a certain layer instead of relying on manually designed architectures.

To our knowledge, we are the first who attempts to combine linear and non-linear embedding propagation in a systematic way, i.e., our gating networks, which can be considered as relay switches, dynamically select between linear GCN and non-linear GCN operations in a layer. This mechanism can be considered as a sort of \emph{neural architecture search} for GCN-based CF. However, our proposed mechanism is much more sophisticated that it because we make decisions for each user/item and the overall GCN architecture can be varied from a certain node's perspective to another node's.

%hybridizes linear/non-linear embedding propagation to make it more flexible usage of two embeddings. Also, we use Gumbel-Softmax to make gating networks learnable.

We conduct performance comparison experiments using NDCG, Recall, and Precision and {\ours} shows the best performance on three benchmark datasets. Also, we define three classes of users/items depending on their preferences on linear GCN and non-linear GCN: FNL (Full-Non-Linearity), PNL (Partial-Non-Linearity), and FL (Full-Linearity). Finally, we analyze the class-specific characteristics of nodes and reveal an important relationship between nodes' roles in a network and their linearity/non-linearity. Contributions of our paper can be summarized as follow: {\begin{itemize}[leftmargin=*]
\item We propose HMLET, which adaptively selects the best propagation layer for a certain node at a certain layer.
\item We demonstrate the effectiveness of HMLET by showing that it marks the best accuracy in all three benchmark datasets.
\item We conduct in-depth analyses to show how linearity or non-linearity of nodes are decided.
\end{itemize}}


==> sec-method.tex <==
\section{Proposed Approach}\label{sec:method}
% \usepackage{tabularx} % <-- new

\begin{figure*}
  \centering
  \includegraphics[width=\textwidth]{img/overview.pdf}
  \caption{Overview of \ours. One can consider our gating network as a relay switch between linear and non-linear layers. While calculating an embedding for a user or an item, therefore, our gating network learns the optimal selection providing the best prediction accuracy, e.g., it selects linear $\rightarrow$ non-linear $\rightarrow$ linear for some user or item while it selects a totally different sequence for other user or item.}\label{overview}
\end{figure*}

In this section, we propose our method \ours. Its key concept is to adopt gating between linear and non-linear propagation layers. In other words, we prepare both linear and non-linear propagation layers but let our gating network with the Gumbel-Softmax decide which one to use in each layer. Table~\ref{table:notations} summarizes a list of notations used in this paper and Figure~\ref{overview} illustrates an overview of \ours.
Specifically, given a user-item pair $(u,v)$, \ours\ first builds a dense embedding of the user $u$ (resp. the item $v$) through the embedding layer (Section 3-1).
After that, the embedding of the user $u$ (resp. the item $v$) is propagated to its neighbors through propagation layers (Section 3-2-1).
Here, \ours\ selects either a linear or a non-linear embedding in consideration of  inherent characteristics with respect to the user $u$ (resp. the item $v$) in each layer (Section 3-2-2). 
To this end, we use a gating network based on the Gumbel-Softmax to select a better embedding for each user/item between linear and non-linear ones. 
The Gumbel-Softmax learns an optimal categorical distribution about the selection and lets the gating network select correctly between the linear and non-linear embedding propagation.
In order to predict each user's preference on each item, the user embedding and item embedding selected by the gating network in each layer is aggregated and we perform their dot-product for prediction.

\begin{table}[t]
    \caption{Notations used in this paper}
    \small
    \centering
    \renewcommand{\arraystretch}{1.7}
    \begin{tabular}{c|l}
        \toprule
        \textbf{Notation}                 & \textbf{Description}    \\
        \midrule
        $k$, $k'$, $k''$  & number of layers for liner, non-linear, and gating network \\
        \hline
        $\bm{e}_{u}^{L^l_{i}}$, $\bm{e}_{v}^{L^l_{i}}$     & $u$'s, $v$'s embedding at $i$-th linear layer      \\
        \hline
        $\bm{e}_{u}^{L^n_{i}}$, $\bm{e}_{v}^{L^n_{i}}$       & $u$'s, $v$'s embedding at $i$-th non-linear layer  \\
        \hline
        $\bm{e}_{u}^{L^g_{i}}$, $\bm{e}_{v}^{L^g_{i}}$        & $u$'s, $v$'s embedding selected by gating network at $i$-th layer\\
        \hline
        $d$    & size of embedding dimension    \\
        \hline
        $m$, $n$    & the number of users/items     \\
        \hline
        $\hat{r}_{uv}$    & user $u$'s final preference on item $v$    \\
        \hline
        $\mathcal N_u$, $\mathcal N_v$    & set of items rated by user $u$ and users who rated item $v$ \\
        \bottomrule
    \end{tabular}
    \label{table:notations}
\end{table}

\subsection{Embedding Layer}\label{subsec:embedding}

First, \ours\ represents users (resp. items) as latent vectors through the embedding layer. 
As shown in Figure~\ref{fig:embedding}, we define the embedding layer for users and items as a selection over $\bm{P}\in \mathbb{R}^{m\times d}$ and $\bm{Q}\in \mathbb{R}^{n\times d}$, respectively. 
Given a one-hot vector of a user $\bm{u}$ (resp. an item $\bm{v}$), the embedding layer maps it into a row of $\bm{P}$ (resp. $\bm{Q}$), yielding an embedding $\mathbf e_u$ (resp. $\mathbf e_v$).

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{img/embedding.pdf}
    \caption{Embedding Layer.}\label{fig:embedding}
\end{figure}

%% Insert the formation of Linear GCN, Non-linear GCN 

\subsection{Propagation Layer}\label{sec:model-prop}
\ours\ propagates the embedding $e_u$ (resp. $e_v$) of each user $u$ (resp. item $v$) through propagation layers. 
In this subsection, we describe the propagation process. Eq.~\eqref{eqn:propagate} describes the process of capturing high-order proximity. 
In Section 3-2-1, we formally define the linear-GCN and non-linear-GCN used in this paper.
In Section 3-2-2, we present our gating network that appropriately selects between them in each layer.

\subsubsection{\bfseries{Graph convolution}}
% \paragraph{\textbf{Graph convolution}}
First, embedding vectors are aggregated (AGG) as follows:
\begin{equation}
    \label{eqn:propagate}
    \begin{split}
    \bm{e}_{u}^{L_{i+1}} = AGG( \bm{e}_u^{L_i}, \lbrace \bm{e}_v^{L_i}: v\in \mathcal N_u \rbrace,\\
    \bm{e}_{v}^{L_{i+1}} = AGG( \bm{e}_v^{L_i}, \lbrace \bm{e}_u^{L_i}: u\in \mathcal N_v \rbrace).
    \end{split}
\end{equation}
where $\bm{e}_u^{L_i}$ and $\bm{e}_v^{L_i}$ indicate user $u$'s embedding and item $v$'s embedding at $i\text{-th}$ layer, respectively. 
That is, $(i+1)\text{-th}$ layer updates $u$'s embedding $\bm{e}_u^{L_{i+1}}$ by aggregating the embeddings of $u$ and $v$ rated by $u$ from $i\text{-th}$ layer.
Similarly, we do the same thing for $\bm{e}_v^{L_{i+1}}$.

Recently, a linear GCN~\cite{He20LightGCN} has been proposed to solve the over-smoothing problem of a non-linear GCN by removing a feature transformation and non-linear activation functions, and it shows better performance than existing non-linear GCN. In \ours, we adopt the linear layer definition of \light. The linear embedding propagation of \light\ is performed as follows:
\begin{equation}
    \begin{split}
    \bm{e}_{u}^{L^l_{i+1}} = \mathop{\mathlarger{\sum}}_{v\in  \mathcal N_u} \frac{1}{\sqrt{\vert \mathcal N_u \Vert \mathcal N_v \vert}} \bm{e}_{v}^{L^l_{i}},\\
    \bm{e}_{v}^{L^l_{i+1}} = \mathop{\mathlarger{\sum}}_{v\in \mathcal N_v} \frac{1}{\sqrt{\vert \mathcal N_v \Vert \mathcal N_u \vert}} \bm{e}_{u}^{L^l_{i}}.
    \end{split}
\end{equation}
where $\bm{e}_{u}^{L^l_{i}}$ and $\bm{e}_{v}^{L^l_{i}}$ indicate user and item embeddings at $i\text{-th}$ layer by \light, respectively. $\frac{1}{\sqrt{\vert \mathcal N_u \Vert \mathcal N_v \vert}}$ is a symmetric normalization term that prevents the scale of embedding from increasing as propagation goes on.

For non-linear embedding propagation, we design a variant of linear embedding propagation of \light\ by adding a non-linear activation function. Its propagation is preformed as follows:
\begin{equation}
    \begin{split}
    \bm{e}_{u}^{L^n_{i+1}} = \phi ( \mathop{\mathlarger{\sum}}_{v\in \mathcal N_u} \frac{1}{\sqrt{\vert \mathcal N_u \Vert \mathcal N_v\vert }}  \bm{e}_{v}^{L^n_{i}} ),\\
    \bm{e}_{v}^{L^n_{i+1}} = \phi ( \mathop{\mathlarger{\sum}}_{v\in \mathcal N_v} \frac{1}{\sqrt{\vert \mathcal N_v \Vert \mathcal N_u\vert }}  \bm{e}_{u}^{L^n_{i}} ).
    \end{split}
\end{equation}
where $\phi$ is a non-linear activation (e.g., ELU, Leaky ReLU, etc.). 

Note that \ours\ use both the linear and non-linear GCN intercorrelated through gating networks which will be described in next subsection.
% Therefore, we can employ any GCN models under \ours\ (\ie\ model-agnostic). 
% In this sense, when a \textit{linear/non-inear GCN} with better performance are available, \ours\ can simply replace the current GCN with that model, thereby improving the accuracy of recommendation.

\subsubsection{\bfseries{Gating network}}
% \paragraph{\textbf{Gating network}} 
Now, we have the linear and non-linear embeddings obtained from $i\text{-th}$ layer.
In this case, as mentioned earlier, linear or non-linear features may coexist in user-item interactions.
Therefore, we should appropriately select linear/non embedding that represents latent space of each user/item.
Toward this end, we design a gating network that adaptively selects either a linear or non-linear embedding by analyzing inherent characteristics of a given user or item.

Figure~\ref{fig:gating} shows the overall architecture of our gating network.
In the case of users, given both the linear and non-linear embeddings, denoted $\bm{e}_{u}^{L^l_{i}}$ and $\bm{e}_{u}^{L^n_{i}}$, respectively, of a user $u$, our gating network selects the best one, denoted as $\mathbf e_{u}^{L^g_{i}}$, and then propagate it to next layer.
Similarly, the gating network selects the best embedding propagation for each item.
% Note that \ours\ here selects one embedding each from every layer, rather than the specific layers.
The intuition behind this technique is that the embedding of each user (resp. item) may consist of both linear and non-linear components.
We formally define the process of performing the gating network in each layer as follows:
\begin{equation}
    \begin{split}
        \bm{g} &= \text{GN}(\bm{e}_{u}^{L^l_{i}},\bm{e}_{v}^{L^l_{i}},\bm{e}_{u}^{L^n_{i}},\bm{e}_{v}^{L^n_{i}}), \\
        \bm{e}_{u}^{L^g_{i}},\bm{e}_{v}^{L^g_{i}} &= \bm{g} \cdot \; \text{stack}(\bm{e}_{u}^{L^l_{i}},\bm{e}_{v}^{L^l_{i}},\bm{e}_{u}^{L^n_{i}},\bm{e}_{v}^{L^n_{i}}),
    \end{split}
\end{equation}
where GN indicates the gating network in Algorithm ~\ref{alg:gating}. The input embeddings are concatenated and then passed to a MLP (multi-layer perceptron). The result of the MLP is a logit vector $\bm{l}$, an input for the STGS.
The logit vector $\bm{l}$ corresponds to $\log \bm{\pi} $ explained in Section~\ref{subsec:gumbel}. $\bm{g}$, the output of GN, represents a linear or non-linear selection by the gating network.
The finally selected embedding $e_u^{L_{i}^g }$, $e_v^{L_{i}^g }$ by the gating network can be calculated by the dot-product at the end.

\begin{algorithm}[t]
  \small
  \DontPrintSemicolon
  \SetAlgoLined
  \KwIn{User and item embeddings}
  \SetKwFunction{FMain}{GN}
  \SetKwProg{Fn}{Function}{:}{}
  \Fn{\FMain{ $\bm{e}_{u}^{L_i^l}, \bm{e}_{v}^{L_i^l}, \bm{e}_{u}^{L_i^n}, \bm{e}_{v}^{L_i^n}$}}{
        $\bm{e}_{\text{concat}} \gets [ \bm{e}_{u}^{L_i^l}, \bm{e}_{v}^{L_i^l}, \bm{e}_{u}^{L_i^n}, \bm{e}_{v}^{L_i^n} ]$ \\
        $\bm{l} \gets $\text{MLP}$(\bm{e}_{\text{concat}})$\; \\
        $\bm{g} \gets $\text{STGS}$(\bm{l}, \tau)$\; \\
  }
  \KwRet $\bm{g}$\;
  \caption{Gating Network}\label{alg:gating}
\end{algorithm}

 \begin{figure}[t]
     \centering
     \includegraphics[width=0.8\columnwidth]{img/gating3.pdf}
     \caption{The overall architecture of our gating network.}\label{fig:gating}
 \end{figure}

% Given both $\mathbf(e_{u}^{L^l_{i}}$ (resp. $e_{v}^{L^l_{i}}$) and $\mathbf (e_{u}^{L^n_{i}},e_{v}^{L^n_{i}})$ of a user $u$ 
% at $i$-th layer, our gating network selects a embedding, $\mathbf(e_{u}^{L^g_{i}},e_{v}^{L^g_{i}})$ , through the gating network, 
% % which is the output embedding $\mathbf(e_{u}^{L^l_{i}},e_{v}^{L^l_{i}})$, $\mathbf (e_{u}^{L^n_{i}},e_{v}^{L^n_{i}})$ of each $i-$th layer. 
% The selected embedding $\mathbf(e_{u}^{L^g_{i}},e_{v}^{L^g_{i}})$ is used as the input of the next $(i+1)\text{-th}$ layer. The intuition behind this model is that the embedding of each user (resp. item) is that different features(linear or non-linear) are aggregated and updated for each $i-$hop neighbor.


However, in the case of non-linear layers, an over-smoothing problem occurs when the number of layers is large. 
To address this problem, we further design variants of the gating network, which can be used when the number of linear layers is more than the number of non-linear layers.
As shown in Figure \ref{fig:types}, there can be three variants, denoted as \ourf, \ourm, and \oure,  depending on the location of the non-linear layer. 
% Each of the variants is presented in .
Specifically, \ourf, \ourm, and \oure\ employ the gating network at initial layers, middle layers, and last layers, respectively. 
First, \ourf\ focuses on the fact that GCNs are highly influenced by near neighborhood~\cite{tang15line}, such as 1-hop and 2-hop neighbors. 
Therefore,  \ourf\ performs the gating network in the front and then only uses the linear propagation layer.
% can be learned by selecting embedding better than linear embedding in the beginning. 
%Figure \ref{fig:types}-Type C is a model that reinforces embedding by using the embedding of a linear model that has been proven to have good performance for the initial embedding and the last embedding, and selecting linear embedding and non-linear embedding in the middle. 
Next, \ourm\ only uses linear embedding with good performance in the front and then performs the gating network at the end.
% Finally, Figure \ref{fig:types}-Type D, linear embedding with good performance is used for initial embedding, and linear embedding and non-linear embedding are selected only at the end. 
The intuition behind \oure\ is that we fine-tune embeddings learned by linear layers at the end --- our experiments and analyses show that \oure is the best among the three variations of the proposed method. The algorithm of our most effective \oure\ is in Algorithm~\ref{algo:type_d}.
% It can be said that fine-tuning was performed using the \textit{non-linear GCN} in the \textit{linear GCN}.
%\textit{linear GCN} with good performance is used, and the non-linear model and the linear model are considered together at the end, further reinforcing embedding that is not well learned in the linear model. That is, it is the same as learning through a linear model and fine-tuning using a non-linear model.

\begin{figure}[H]
    \centering
    \includegraphics[width=\columnwidth]{img/types.pdf}
    \caption{Three variants of our gating network.}\label{fig:types}
\end{figure} 

% Among the variants, we predict that the \ourm\ that reinforces embedding by using a \textit{linear GCN} with good performance at the beginning and a \textit{non-linear GCN} at the last embedding will be the best. 
% In Section~\ref{sec:eval}, we confirm that \ourm\ is the most effective in terms of recommendation accuracy, compared to other variants.

\input{algorithm_hmlet_end}

\subsection{Prediction Layer}\label{subsec:prediction}
After propagating through all $k$ layers, we predict each user's preference for each item. To this end, we create a dot-product value of the selected embeddings by our gating network in each layer and use the residual prediction as follows:
\begin{align}\begin{split}\label{eq:aaa}
    \hat{r}^{i}_{uv} =& \; \mathbf  e_{u}^{L_{i}} \odot \mathbf  e_{v}^{L_{i}},\\
    \hat{r}_{uv} =& \mathop{\mathlarger{\sum}}^k_{i=0} \hat{r}^{i}_{uv}.
\end{split}\end{align}
In the previous GCN-based recommendation system research, only the last embedding was used to predict, but in \ours, the above residual prediction $\hat r_{uv}$ is used. This residual prediction can produce good performance by using not only the last embedding but also the early embedding.
In summary, \ours\ predicts users' preferences on the items by considering both linear embedding and non-linear embedding based on the residual prediction.
% and all hops.

\subsection{Training Method}\label{subsec:opt}

For training \ours, we employ the Bayesian personalized ranking (BPR) loss, denoted $L$, which is popularly used in many CF method\cite{Rendle09BPR}. 
The BPR loss is as follows:
% \begin{equation}
%     \begin{split}
%     \mathbf L(R,\hat{R}) = - \mathop{\mathlarger{\sum}}^M_{a=1} \mathop{\mathlarger{\sum}}_{ (i,j) \in D_a} \ln \sigma(\hat{r}_{ai} - \hat{r}_{aj}) + \lambda\lVert \mathbf{\Theta_1} \rVert ^2,
%     \end{split}
% \end{equation}

\begin{equation}
    \begin{split}
    \mathbf L(R,\hat{R}) = - \mathop{\mathlarger{\sum}}^M_{u=1} \mathop{\mathlarger{\sum}}_{i\in N_u} \mathop{\mathlarger{\sum}}_{j\notin N_u}  \ln (\sigma(\hat{r}_{ui} - \hat{r}_{uj})) + \lambda\lVert \mathbf{\Theta_1} \rVert ^2
    \end{split}
\end{equation}
where $\sigma$ is the sigmoid function. $ \Theta_{1}$ is the embedding of the $0-$th layer, and $\lambda$ controls the $L_2$ regularization strength. We use each observed user-item interaction as a positive instance and then conduct the negative sampling strategy. 

Also, we employ STGS for smooth optimization of the gating network. We can train the network with annealing temperature, and we use the temperature decay for each epoch. Furthermore, we train a model that shows outstanding performance through the optimal temperature range and decay value.



% $ D_a = \{ (i,j) \vert i \in R_{a} \land j \in V-R_{a} \} $ denotes the pairwise training data for $a$ with $R_a$ represents the itemset that $a$ positively shows feedback. 

==> sec-relatedwork.tex <==
\section{Related Work}\label{sec:related}
In this section, we briefly review traditional recommender systems including GCN-based methods and present Gumbel-Softmax used in our proposed methods.

\subsection{Recommender Systems}
Traditional recommender systems have focused on matrix factorization (MF) techniques ~\cite{Koren09MF}. Typical MF-based methods include BPR~\cite{Rendle09BPR} and WRMF~\cite{Hu08WRMF}. These MF-based methods simply learn relationships between users and items via dot products. Therefore, they have limitations in considering potential complex relationships between users and items inherent in user-item interactions~\cite{He17NeuMF}. To overcome these limitations, deep learning (DL) (e.g., Autoencoder \cite{kingma2013auto,rezende2014stochastic}, graph convolutional networks (GCNs)~\cite{Bruna2014,Defferrard2016,kipf2017semi,Wu2019SGC,Atwood2015,Gilmer2017,Hamilton2017,Velickovic2018,Gao2018}) based recommender systems have been proposed in recommendation domains to effectively learn those non-linear relationships between users and items ~\cite{Wang19NGCF,Ying18pinsage,liu08eigenrank,Rianne17GCMC}.

Recently, recommender systems~\cite{Wang19NGCF,Ying18pinsage,Rianne17GCMC} using GCNs are getting much attention. GCN-based methods can effectively learn the behavioral similarity between users and items by 'directly' capturing the collaborative signals inherent in user-item interactions~\cite{Wang19NGCF}. Typical GCN-based methods include GC-MC~\cite{Rianne17GCMC}, PinSage~\cite{Ying18pinsage}, and NGCF~\cite{Wang19NGCF}.

Generally, GCN-based methods model user-item interactions as a user-item bipartite graph and then perform the following three steps:

{\bfseries (Step 1) Embedding Layer:} We randomly set the initial embedding $e^0$ of all users $u$ and items $v$.
\begin{equation}
    \begin{split}
    \mathbf  e_{u}^{0}, e_{v}^{0} \in \mathbb {R}^{d}
    \end{split}
\end{equation}
where $d$ denotes the embedding size.

{\bfseries (Step 2) Propagation Layer:} Given $k$ layers, the embedding of a user node $u$ (resp. an item node $v$) in $i$-th (i.e., 1≤$i$≤$k$) layer is updated based on the embeddings of $u$ (resp. $v$) and its neighbors $N_u$ (resp. $N_v$) in ($i$-1)-th layer.

\begin{equation}
    \begin{split}
    \mathbf  e_{u}^{i} = \sigma ( \Sigma_{v\in N_u} e_v^{i-1} W_{i-1} ), \\
    \mathbf  e_{v}^{i} = \sigma ( \Sigma_{u\in N_v} e_u^{i-1} W_{i-1} ).
    \end{split}
\end{equation}

where $\sigma$ denotes a non-linear activation function (e.g., $ReLU$), and $W_{i-1}$ is a trainable transformation matrix. Some methods also include a self-embedding in the ($i$-1)-th layer (i.e., $e_{u}^{i-1}$ or $e_{v}^{i-1}$, respectively) during the aggregation process.

{\bfseries (Step 3) Prediction Layer:} The preference of user $u$ for item $i$ is predicted using the dot-product between the user $u$ and item $i$ embeddings of the last layer $k$ (i.e., $e_{u}^{k}$ and $e_{v}^{k}$).

\begin{equation}
    \begin{split}
    \hat{r}_{uv} = e_{u}^{k} \odot e_v^k
    \end{split}
\end{equation}

However, these GCN-based methods have two limitations: (L1) Training Difficulty ~\cite{Wu2019SGC,Chen20LRGCCF,He20LightGCN} and (L2) Over-Smoothing (i.e., indistinguishable embeddings of nodes) ~\cite{chen2020measuring,li2018deeper}. First, (L1) is caused by their ~\cite{Rianne17GCMC,Ying18pinsage,Wang19NGCF} use of a non-linear activation function in the propagation step. Specifically, the non-linear operation of the activation function complicates the propagation layer step and furthermore this operation is repeatedly performed whenever a layer is stacked over. Thus, they suffer from training difficulty with non-linear activation functions for large-scale user-item bipartite graphs ~\cite{Wu2019SGC,chen2020measuring,li2018deeper}.

Next, (L2) is caused as they ~\cite{Rianne17GCMC,Ying18pinsage,Wang19NGCF} use only the embeddings updated through the last layer in the prediction layer. Specifically, as the layer becomes deeper, the embedding of each node will receive more of the embeddings of its neighborhood. As a result, the embedding of each node in the last layer becomes similar to the embedding of many directly/indirectly connected nodes, resulting in the loss of uniqueness~\cite{Chen20LRGCCF,chen2020measuring,li2018deeper}. This phenomenon prevents traditional GCN-based methods from effectively utilizing information of high-order neighborhood. Empirically, this is also shown by the fact that many GCN-based methods show better performance when using only two layers than using more than two.

Recently, LR-GCCF~\cite{Chen20LRGCCF} and LightGCN~\cite{He20LightGCN}, which are GCN-based recommender systems to alleviate both (L1) and (L2), have been proposed. First, to alleviate (L1), they perform linear embedding propagation without using a non-linear activation function in the propagation layer step. Also, to mitigate (L2), they aggregate the embeddings of the last layer as well as the embeddings of all other earlier layers for prediction. After that, they perform residual predictions~\cite{Chen20LRGCCF, He20LightGCN}, which predict each user's preference for each item based on the aggregated embedding. In~\cite{Chen20LRGCCF,He20LightGCN}, the authors demonstrated that a GCN structure with linear embedding propagation and residual prediction can significantly improve the recommendation accuracy by successfully addressing (L1) and (L2).

\begin{table*}
  \caption{GCN-based Recommender Systems}
  \label{tab:GCNs}
  \begin{tabular}{ccccccc}
  \toprule
  & GC-MC~\cite{Rianne17GCMC} & PinSage~\cite{Ying18pinsage} & NGCF\cite{Wang19NGCF} & LR-GCCF~\cite{Chen20LRGCCF} & LightGCN\cite{He20LightGCN} & \textbf{Ours}
\\ \midrule
Non-Linear Embedding Propagation & O & O & O & X & X & O \\
Linear Embedding Propagation & X & X & X & O & O & O \\
Residual Prediction & X & X & O & O & O & O\\
\bottomrule
\end{tabular}
\end{table*}

In summary, GCN-based recommender systems can be categorized by, as shown in Table \ref{tab:GCNs}, propagation and prediction methods. Here, we note that they consider only one of the linear/non-linear characteristics of user-item interactions. However, we conjecture that user-item interactions are neither only linear nor only non-linear, for which we will conduct in-depth analyses in Section~\ref{sec:analysis}. Therefore, in this paper, we propose a \textbf{H}ybrid \textbf{M}ethod of \textbf{L}inear and non-lin\textbf{E}ar collaborating fil\textbf{T}ering method (\ours, pronounced as Hamlet), which consider both two disparate characteristics for selecting proper embedding propagation every layer.
\subsection{Gumbel-Softmax}\label{subsec:gumbel}
The Gumbel-max trick \cite{Gumbel54,Maddison14sampling} provides a way to sample a one-hot vector from a categorical distribution with class probabilities $\bm{\pi}$:
\begin{equation}
    \label{eqn:Gumbel-max}
   \bm{z}=one\_hot(\arg \max\limits_{\substack{i}}[g_i+log\pi_i])
\end{equation}
where $g_1...g_k$ are samples drawn from the unit Gumbel distribution $Gumbel(\bm{0},\bm{1})$. The argmax operator prevents gradients flowing through the Gumbel-max, because it gives zero gradients irrespective of how $\pi$ was created, which loss function is used, and so on. To this end, the Gumbel-Softmax~\cite{jang16categorical} function generates a sample $\bm{y}$ that approximates $\bm{z}$ via the reparameterization trick defined as follow:
\begin{equation}
    \label{eqn:Gumbel-Softmax}
    y_i=\frac{\exp \left(\left(\log \left(\pi _i\right)+g_i\right)/\tau \right)}{\sum _{j=1}^k\exp \left(\left(\log \left(\pi _j\right)+g_j\right)/\tau \right)}
\end{equation}
where $y_i$ is $i-$th component of the vector $\bm{y}$, and $\tau$ is a temperature that determines how closely the function approximates the sample $\bm{\pi}$. However, the Gumbel-Softmax is challenging to use if it needs to be sampled into discrete values because, when the temperature is high, the Gumbel-Softmax output is not categorical. To solve this problem Straight-Through Gumbel-Softmax (STGS) can be used. STGS always generates discrete outputs while letting the gradients flow through $y_i$, even when the temperature is high. This makes the network learnable while annealing the temperature.

This Gumbel-Softmax has been widely used to learn optimal categorical distributions. One such example is \emph{network architecture search (NAS)} ~\cite{hu2020neural,wan2020fbnetv2,chang2019differentiable,wu2019fbnet,he2020milenas,xie2018snas,li2020neural,hu2020dsnas}. In NAS, we let an algorithm find optimal operators (among many pre-determined candidates prepared by user) and their connections. All these processes can be modeled by generating optimal one-hot (or multi-hot) vectors and the Gumbel-Softmax is used~\cite{jang16categorical}. Another example is a multi-generator-based generative adversarial networks (GANs). Park et al. showed that a data is typically multi-modal, and it is necessary to separate modes and assign a generator to each mode of data, e.g., one generator for long-hair female, another generator for short-hair male and so on for a GAN generating facial images~\cite{Park2018}. In our case, we try to separate the two modes, i.e., linear and non-linear characteristics, of the user-item interaction bipartite graph.
